Jais 2: A Family of Arabic-Centric Open Large Language Models

Jais 2 is a family of Arabic-centric large language models developed jointly by MBZUAI, Cerebras, and Inception, designed to advance Arabic-centric language modeling, with strong performance across the Arabic and culturally grounded benchmarks evaluated in this report. The family includes, to our knowledge, the largest open Arabic-centric LLM trained from scratch at 70B parameters, and a competitive 8B-parameter variant among the evaluated open models. A custom Arabic-centric vocabulary enables efficient training and inference. In addition, an optimized architecture and training recipe yield highly compute-efficient training. With a substantially smaller token budget than comparable models, Jais 2 achieves strong Arabic performance on the benchmarks considered in this report and competitive English results. The models obtain leading results among the evaluated open models on OALL2 and AraGen. They also perform strongly on several culturally grounded Arabic benchmarks, including poetry, religion, cuisine, and dream interpretation, as well as in general tasks such as translation and summarization. We release the models in HuggingFace under a commercially permissive license. Jais 2 70B is also released as a chat app on the Web, iOS, and Android; it runs on Cerebras hardware, delivering up to 2,000 tokens per second, and enabling high-throughput Arabic-centric chat serving in our deployment setting. By uniting scale, linguistic diversity, cultural fidelity, openness, and speed, Jais 2 provides an open-weight foundation intended to support further research and development in Arabic-centric LLMs.

==> Tables/dialect_id_results_madar.tex <==
\begin{table*}[h!]
\centering
\setlength{\tabcolsep}{2.8pt}      % Compact column padding to fit all columns
\renewcommand{\arraystretch}{1.1}  % Moderate row height
\resizebox{\textwidth}{!}{%        % Resize to fit the text width
\begin{tabular}{lrrrrrrrrrrr}
\toprule
\textbf{Model} & \textbf{acm} & \textbf{aeb} & \textbf{afb} & \textbf{apc} & \textbf{apd} & \textbf{ar} & \textbf{arq} & \textbf{ars} & \textbf{ary} & \textbf{arz} & \textbf{AVG} \\
\midrule
\multicolumn{12}{l}{\textbf{Open models $\leq$ 13B parameters}} \\
\midrule

\model{jais-adapted-13b-chat} & 2.06 & 44.94 & 50.25 & 23.19 & 5.72 & 73.92 & 9.48 & 6.42 & 66.70 & 36.68 & 31.94 \\
\model{jais-family-13b-chat} & 7.07 & 28.80 & 68.91 & 30.02 & 5.62 & 49.45 & 26.42 & 20.65 & 46.95 & 55.08 & 33.90 \\
\model{jais-family-6p7b-chat} & 10.28 & 41.58 & 63.53 & 35.19 & 18.91 & 68.42 & 6.67 & 23.01 & 23.69 & 39.97 & 33.13 \\
\model{jais-adapted-7b-chat} & 1.55 & 10.58 & \textbf{83.67} & 30.89 & 2.51 & 46.40 & 9.71 & 3.39 & 10.60 & 26.76 & 22.61 \\
\model{gemma-3-12b-it} & 32.35 & 41.58 & 29.31 & 38.31 & 14.19 & 59.01 & \textbf{58.11} & 9.07 & 72.19 & 56.19 & 41.03 \\
\model{gemma-3-4b-it} &\textbf{ 36.76} & 39.26 & 27.17 & 6.11 & 20.86 & 20.27 & 24.68 & 4.26 & 54.52 & 50.55 & 28.44 \\
\model{gemma-2-9b-it} & 8.02 & 17.59 & 38.20 & 22.11 & 8.07 & 66.12 & 21.53 & 8.76 & \textbf{77.61} & 84.01 & 35.20 \\
\model{Qwen3-8B} & 29.74 & 35.74 & 41.38 & 7.86 & 1.45 & \textbf{91.44} & 31.02 & 4.62 & 34.98 & 67.37 & 34.56 \\
\model{Qwen2.5-7B-Instruct} & 14.39 & 17.08 & 29.77 & 35.11 & 17.40 & 45.15 & 33.06 & 7.27 & 59.84 & 63.61 & 32.27 \\
\model{Llama-3.1-8B-Instruct} & 9.78 & 23.88 & 60.34 & 9.78 & 12.54 & 66.42 & 14.36 & 18.23 & 31.83 & 78.64 & 32.58 \\
\model{ALLaM-7B-Instruct-preview-v2} & 11.48 & \textbf{53.76} & 29.41 & 69.74 & 8.07 & 71.07 & 41.33 & 22.83 & 67.87 & 85.94 & \textbf{46.15} \\
\model{Fanar-1-9B-Instruct} & 13.19 & 20.65 & 26.22 & 54.68 & 15.30 & 79.08 & 27.09 & 12.35 & 77.05 & \textbf{93.56} & 41.92 \\
\model{Falcon-H1-7B-Instruct} & 11.53 & 20.44 & 49.92 & 25.40 & 12.99 & 58.36 & 20.91 & 9.35 & 49.06 & 88.18 & 34.61 \\
\model{aya-23-8B} & 9.78 & 19.04 & 40.93 & 14.44 & 16.25 & 28.03 & 8.48 & 33.87 & 21.02 & 71.11 & 26.30 \\
\model{aya-expanse-8b} & 5.92 & 41.04 & 19.77 & 37.54 & 17.20 & 38.09 & 21.84 & 20.49 & 69.22 & 88.42 & 35.95 \\
\model{Yehia-7B-preview} & 8.17 & 28.58 & 32.92 & 71.24 & 16.15 & 57.66 & 26.31 & 24.76 & 75.11 & 83.73 & 42.46 \\
\model{c4ai-command-r7b-12-2024} & 6.97 & 43.77 & 29.82 & \textbf{87.62} & 17.75 & 52.65 & 20.30 & 12.63 & 55.36 & 69.07 & 39.59 \\
\model{AceGPT-v2-8B-Chat} & 9.03 & 20.88 & 61.53 & 23.96 & \textbf{21.51} & 94.79 & 14.82 & 9.09 & 65.58 & 71.99 & 39.32 \\
\model{Hala-9B} & 10.33 & 34.72 & 15.29 & 26.72 & 14.69 & 39.24 & 27.72 & 11.17 & 69.32 & 88.96 & 33.82 \\
\model{SILMA-9B-Instruct-v1.0} & 13.14 & 22.05 & 39.73 & 19.58 & 6.87 & 19.92 & 35.22 & 13.43 & 69.78 & 72.86 & 31.26 \\
%Changed to new numbers by Hakim
%\st{Jais-2-8B (ours)} & 19.46 & 18.28 & 22.35 & 45.05 & 11.74 & 84.63 & 20.35 & 74.11 & 38.94 & 74.05 & 40.90 \\
\model{Jais-2-8B (ours)} & 27.13 & 31.48 & 41.09 & 54.96 & 14.39 & 80.13 & 29.99 & \textbf{44.07} & 50.03 & 87.02 & 46.03 \\
\midrule
\multicolumn{12}{l}{\textbf{Open models $>$ 13B parameters}} \\
\midrule
\model{Jais-2-70B (ours)} & 11.94 & \textbf{74.02} & 60.55 & 73.50 & \textbf{43.38} & 86.19 & \textbf{48.91} & 18.39 & \textbf{90.24} & 91.73 & \textbf{59.89} \\
\model{gemma-3-27b-it} & 11.38 & 51.47 & 56.59 & 58.01 & 25.58 & 71.27 & 31.17 & 13.92 & 82.49 & 92.59 & 49.45 \\
\model{Falcon-H1-34B-Instruct} & 13.99 & 48.79 & 34.77 & 28.76 & 20.01 & 84.23 & 26.01 & 14.97 & 77.61 & 90.29 & 43.94 \\
\model{Qwen2.5-32B-Instruct} & \textbf{19.36} & 32.45 & 50.07 & 47.93 & 17.45 & 90.29 & 29.69 & 21.96 & 73.61 & 85.60 & 46.84 \\
\model{jais-family-30b-16k} & 2.76 & 40.30 & \textbf{86.42} & 57.99 & 1.76 & 85.29 & 37.41 & 7.16 & 47.51 & 67.04 & 43.36 \\
\model{jais-family-30b-8k} & 10.78 & 55.21 & 39.26 & 32.64 & 3.61 & 80.98 & 40.93 & 7.55 & 74.94 & 70.00 & 41.59 \\
\model{Qwen2.5-72B-Instruct} & 17.95 & 31.48 & 55.81 & 72.93 & 4.61 & \textbf{95.20} & 20.08 & 19.75 & 71.20 & \textbf{94.10} & 48.31 \\
\model{Llama-3.1-70B-Instruct} & 17.20 & 29.77 & 40.27 & 87.73 & 14.44 & 86.84 & 24.25 & 9.55 & 66.60 & 67.98 & 44.46 \\
\model{Llama-3.3-70B-Instruct} & 15.70 & 35.20 & 36.93 & \textbf{89.51} & 10.83 & 83.23 & 23.17 & 13.97 & 75.01 & 69.43 & 45.30 \\
\model{jais-adapted-70b-chat} & 4.31 & 63.57 & 48.74 & 50.94 & 7.92 & 83.73 & 39.22 & \textbf{34.13} & 64.01 & 89.03 & 48.56 \\
\bottomrule
\end{tabular}
}
\caption{Model accuracy (\%) on the MADAR Arabic Dialect Identification benchmark. Columns represent specific dialects, Modern standard Arabic (\textbf{ar}), and the average accuracy (\textbf{AVG}) across all subsets.}
\label{tab:dialect_id_results_madar}
\end{table*}

==> Tables/dialect_id_results_qadi.tex <==
\begin{table*}[h!]
\centering
\setlength{\tabcolsep}{2.8pt}      % Compact column padding to fit all columns
\renewcommand{\arraystretch}{1.1}  % Moderate row height
\resizebox{\textwidth}{!}{%        % Resize to fit the text width
\begin{tabular}{lrrrrrrrrrrrr}
\toprule
\textbf{Model} & \textbf{acx} & \textbf{aeb} & \textbf{afb} & \textbf{apc} & \textbf{apd} & \textbf{ar} & \textbf{ars} & \textbf{ary} & \textbf{arz} & \textbf{avb} & \textbf{ayl} & \textbf{AVG} \\
\midrule
\multicolumn{12}{l}{\textbf{Open models $\leq$ 13B parameters}} \\
\midrule
\model{jais-adapted-13b-chat} & 78.00 & 37.00 & 70.10 & 27.85 & 26.00 & 63.00 & 9.50 & 55.00 & 57.00 & 11.50 & 22.00 & 41.54 \\
\model{jais-family-13b-chat} & 24.50 & 26.50 & 71.70 & 30.74 & 25.50 & 45.50 & 21.50 & 40.00 & 68.50 & 30.75 & 16.00 & 36.47 \\
\model{jais-family-6p7b-chat} & 8.00 & 34.50 & 68.10 & 38.64 & 30.00 & 65.50 & 38.50 & 24.00 & 58.00 & 8.75 & 21.00 & 35.91 \\
\model{jais-adapted-7b-chat} & 26.00 & 15.50 & 81.70 & 31.24 & 21.00 & 48.50 & 4.50 & 18.00 & 33.50 & 4.25 & 9.50 & 26.70 \\
\model{gemma-3-12b-it} & 24.50 & 41.00 & 47.20 & 41.41 & 47.50 & 74.50 & 22.00 & 61.50 & 56.00 & 30.25 & 37.50 & 43.94 \\
\model{gemma-3-4b-it} & 6.50 & 34.50 & 38.50 & 7.40 & 46.00 & 37.00 & 3.00 & 46.50 & 55.00 & 19.75 & 14.00 & 28.01 \\
\model{gemma-2-9b-it} & 7.00 & 22.00 & 54.10 & 18.07 & 19.50 & 53.00 & 23.00 & 70.00 & 87.00 & 31.00 & 14.50 & 36.29 \\
\model{Qwen3-8B} & 3.50 & 44.00 & 43.20 & 5.40 & 13.50 & 94.50 & 4.50 & 33.50 & 81.50 & 4.00 & 23.50 & 31.92 \\
\model{Qwen2.5-7B-Instruct} & 24.00 & 25.00 & 34.70 & 34.50 & 33.00 & 75.50 & 11.50 & 46.00 & 86.50 & 14.50 & 10.00 & 35.93 \\
\model{Llama-3.1-8B-Instruct} & 12.00 & 34.00 & 68.40 & 14.81 & 24.00 & 45.50 & 20.50 & 24.50 & 81.00 & 5.00 & 14.00 & 31.25 \\
\model{ALLaM-7B-Instruct-preview-v2} & 38.50 & 45.50 & 56.50 & 54.45 & 31.50 & 82.50 & 30.50 & 60.50 & 91.50 & 28.75 & 30.50 & 50.06 \\
\model{Fanar-1-9B-Instruct} & 4.50 & 26.50 & 47.60 & 49.31 & 34.50 & 73.50 & 28.50 & 65.50 & 94.00 & 31.75 & 18.50 & 43.11 \\
\model{Falcon-H1-7B-Instruct} & 9.50 & 34.50 & 60.80 & 22.08 & 29.00 & 58.50 & 11.50 & 44.00 & 92.50 & 15.00 & 14.00 & 35.58 \\
\model{aya-23-8B} & 10.50 & 28.50 & 43.00 & 15.81 & 32.50 & 28.50 & 38.50 & 22.00 & 76.00 & 21.50 & 25.50 & 31.12 \\
\model{aya-expanse-8b} & 9.50 & 44.00 & 38.30 & 38.77 & 36.50 & 55.00 & 24.00 & 56.50 & 82.50 & 22.50 & 15.50 & 38.46 \\
\model{Yehia-7B-preview} & 41.50 & 31.00 & 51.80 & 62.36 & 44.50 & 62.00 & 36.50 & 61.50 & 89.50 & 17.25 & 25.50 & 47.58 \\
\model{c4ai-command-r7b-12-2024} & 1.50 & 41.00 & 51.60 & 86.07 & 42.00 & 67.50 & 19.50 & 48.00 & 76.00 & 9.75 & 32.50 & 43.22 \\
\model{AceGPT-v2-8B-Chat} & 12.50 & 27.50 & 79.60 & 19.82 & 39.50 & 96.50 & 15.00 & 41.50 & 74.50 & 11.25 & 21.00 & 39.88 \\
\model{Hala-9B} & 11.50 & 44.50 & 37.00 & 24.47 & 35.50 & 44.50 & 30.50 & 56.00 & 86.50 & 20.00 & 17.50 & 37.09 \\
\model{SILMA-9B-Instruct-v1.0 } & 4.00 & 28.00 & 57.80 & 19.95 & 17.00 & 25.00 & 22.50 & 60.50 & 77.00 & 30.75 & 33.00 & 34.14 \\
%Changed by Hakim
%\st{Jais-2-8B (ours)} & 17.00 & 14.50 & 69.40 & 37.89 & 33.00 & 92.00 & 67.50 & 36.50 & 88.00 & 19.50 & 33.50 & 46.25 \\
\model{Jais-2-8B (ours)} & 4.00 & 21.50 & 88.40 & 34.25 & 37.50 & 69.00 & 46.00 & 45.00 & 91.00 & 11.75 & 18.50 & 42.45 \\
\midrule
\multicolumn{12}{l}{\textbf{Open models $>$ 13B parameters}} \\
\midrule
\model{Jais-2-70B (ours)} & 32.00 & 59.00 & 93.10 & 53.07 & 67.50 & 71.50 & 53.50 & 74.00 & 94.50 & 37.00 & 59.50 & 63.15 \\
\model{Falcon-H1-34B-Instruct} & 13.50 & 55.00 & 60.10 & 36.26 & 47.50 & 92.50 & 25.00 & 66.50 & 92.00 & 34.25 & 18.50 & 49.19 \\
\model{Qwen2.5-32B-Instruct} & 24.00 & 29.00 & 63.00 & 55.58 & 46.00 & 83.00 & 29.50 & 49.50 & 94.00 & 12.25 & 12.50 & 45.30 \\
\model{jais-family-30b-16k} & 11.00 & 33.50 & 88.90 & 38.14 & 14.50 & 84.50 & 4.00 & 34.00 & 80.50 & 9.25 & 17.00 & 37.75 \\
\model{jais-family-30b-8k} & 5.50 & 36.50 & 67.70 & 22.58 & 16.50 & 86.00 & 16.00 & 54.50 & 82.00 & 14.25 & 48.00 & 40.87 \\
\model{gemma-3-27b-it} & 15.00 & 41.50 & 69.90 & 59.47 & 57.00 & 75.50 & 29.50 & 69.50 & 94.00 & 15.00 & 30.50 & 50.62 \\
\model{Qwen2.5-72B-Instruct} & 15.00 & 35.50 & 72.80 & 65.37 & 30.50 & 97.50 & 39.50 & 52.50 & 97.00 & 13.00 & 22.50 & 49.20 \\
\model{Llama-3.3-70B-Instruct} & 9.50 & 30.00 & 63.00 & 86.45 & 24.00 & 83.00 & 40.50 & 58.00 & 82.00 & 25.50 & 33.50 & 48.68 \\
\model{Llama-3.1-70B-Instruct} & 12.50 & 28.00 & 64.70 & 85.19 & 25.50 & 89.50 & 28.00 & 54.50 & 79.50 & 21.75 & 29.50 & 47.15 \\
\model{jais-adapted-70b-chat} & 29.00 & 42.00 & 72.90 & 39.52 & 36.50 & 93.50 & 65.50 & 44.50 & 96.50 & 16.25 & 43.00 & 52.65 \\
\bottomrule
\end{tabular}
}
\caption{Model accuracy (\%) on the QADI Arabic Dialect Identification benchmark. Columns represent specific dialects, Modern standard Arabic (\textbf{ar}), and the average accuracy (\textbf{AVG}) across all subsets.}
\label{tab:dialect_id_results_qadi}
\end{table*}

==> Tables/finance_qa.tex <==
% \begin{table}[!ht] 
% \centering
% \small
% \resizebox{\textwidth}{!}{
% \begin{tabular}{lrrrr}
% \toprule
% \textbf{Model} &
% \textbf{Accounting MCQ} &
% \textbf{Arabic Business MCQ} &
% \textbf{Fatwa MCQ} &
% \textbf{Sentiment MCQ} \\
% \midrule


% % ===================== MODELS <= 13B =====================
% \multicolumn{6}{l}{\textbf{Open models $\leq$ 13B parameters}} \\
% \midrule
% % \model{Jais-2-8B} & 33.33 & 67.11 & 67.60 & 42.50 \\
% \model{ALLaM-7B-Instruct-preview-v2} & 25.00 & 69.74 & \textbf{73.60} & 60.00 \\
% \model{Falcon-H1-7B-Instruct}  & 29.17 & 68.42 & 60.40 & 47.50 \\
% \model{Fanar-1-9B-Instruct} & 33.33 & 71.05 & 70.00 & 52.50 \\
% \model{Hala-9B} & 33.33 & 73.68 & 62.00 & 52.50 \\
% \model{SILMA-9B-Instruct-v1.0} & 37.50 & 65.79 & 60.40 & 62.50 \\
% \model{Yehia-7B-preview} & 41.67 & 69.74 & 66.40 & 57.50 \\
% \model{Llama-3.1-8B-Instruct} & 41.67 & 51.32 & \textbf{73.60} & \textbf{67.50} \\
% \model{Qwen2.5-7B-Instruct} & 25.00 & \textbf{76.32} & 65.60 & 47.50 \\
% \model{aya-23-8B} & \textbf{50.00} & 68.42 & 60.40 & 50.00 \\
% \model{aya-expanse-8b} & 12.50 & 47.37 & 63.20 & 65.00 \\
% \model{c4ai-command-r7b-12-2024} & 25.00 & 63.16 & 52.40  & 35.00 \\
% \model{gemma-2-9b-it} & 25.00 & 69.74  & 70.80  & 57.50  \\
% \model{gemma-3-4b-it} & 33.33 & 59.21 & 23.60 & 60.00 \\
% \model{gemma-3-12b-it}  & 37.50 & 69.74 & 72.80 & 57.50 \\
% \model{AceGPT-v2-8B-Chat} & 41.67 & 64.47 & 70.40 & 60.00 \\
% \model{jais-adapted-7b-chat} & 33.33 & 51.32 & 37.60 & 27.50 \\
% \model{jais-family-6p7b-chat} & 16.67 & 39.47 & 20.80 & 47.50 \\
% \model{jais-adapted-13b-chat}  & 33.33 & 61.84 & 64.80 & 42.50 \\
% \model{jais-family-13b-chat}  & 12.50 & 61.84 & 50.80 & 52.50 \\
% \model{Qwen3-8B} & 25.00 & 48.68 & 69.20 & 45.00 \\
% \model{Jais-2-8B} & \abdelaziz{25.00} & \abdelaziz{65.79} & \abdelaziz{62.40} & \abdelaziz{42.50} \\
% \midrule
% \multicolumn{6}{l}{\textbf{Open models $>$ 13B parameters}} \\
% \midrule

% % ===================== MODELS >= 70B =====================
% \model{Jais-2-70B}  & \textbf{\abdelaziz{37.50}} & \abdelaziz{68.42} & \textbf{\abdelaziz{76.80}} & \abdelaziz{42.50} \\
% \model{Llama-3.1-70B-Instruct}  & 20.83 & \textbf{76.32} & 59.20 & 45.00 \\
% \model{Llama-3.3-70B-Instruct}  & 29.17 & 75.00 & 72.80 & 42.50\\
% \model{Qwen2.5-72B-Instruct}  & 25.00 & \textbf{76.32} & 65.60 & \textbf{47.50} \\
% \model{jais-adapted-70b-chat}  & 29.17 & 61.84 & 60.00 & 40.00 \\
% \model{Qwen2.5-32B-Instruct}  & 16.67 & 72.37 & 66.80 & 47.50 \\
% \model{gemma-3-27b-it}  & 33.33 & 71.05 & 65.60 & 55.00 \\
% \model{jais-family-30b-8k-chat}  & 20.83 & 75.00 & 48.40 & 50.00 \\
% \model{jais-family-30b-16k-chat}  & 16.67 & 68.42 & 62.80 & 42.50 \\
% \model{Falcon-H1-34B-Instruct}  & 33.33 & \textbf{76.32} & 71.20 & 60.00 \\
% \bottomrule
% \end{tabular}
% }
% \caption{Performance of various LLMs on the SAHM Arabic Financial Benchmark, reporting accuracy (\%) across four MCQ tasks: Accounting, Business, Fatwa reasoning, and Financial Sentiment. Models are grouped by size ($\geq$70B vs $<$70B) to highlight performance trends across large and mid-size architectures. Jais2 models demonstrate consistent state-of-the-art results across both tiers.}
% \label{tab:financial-mcq}
% \end{table}



\begin{table*}[t]
\centering
\scriptsize
\setlength{\tabcolsep}{2.5pt}
\resizebox{\textwidth}{!}{

\begin{tabular}{l *{4}{c} c}
\toprule
\textbf{Model} & \textbf{Accounting (MCQ)} & \textbf{Arabic Business (MCQ)} & \textbf{Fatwa (MCQ)} & \textbf{Sentiment Analysis (MCQ)} & \textbf{Avg} \\


\midrule
\textbf{Open models $\leq$ 13B parameters} \\
\midrule
\model{gemma-3-12b-it} & 37.50 & 69.74 & 72.80 & 57.50 & \textbf{59.38} \\
\model{AceGPT-v2-8B-Chat} & 41.67 & 64.47 & 70.40 & 60.00 & 59.14 \\
\model{Yehia-7B-preview} & 41.67 & 69.74 & 66.40 & 57.50 & 58.83 \\
\model{Llama-3.1-8B-Instruct} & 41.67 & 51.32 & \textbf{73.60} & \textbf{67.50} & 58.52 \\
\model{aya-23-8B} & \textbf{50.00} & 68.42 & 60.40 & 50.00 & 57.21 \\
\model{ALLaM-7B-Instruct-preview} & 25.00 & 69.74 & \textbf{73.60} & 60.00 & 57.08 \\
\model{Fanar-1-9B-Instruct} & 33.33 & 71.05 & 70.00 & 52.50 & 56.72 \\
\model{SILMA-9B-Instruct-v1.0} & 37.50 & 65.79 & 60.40 & 62.50 & 56.55 \\
\model{gemma-2-9b-it} & 25.00 & 69.74 & 70.80 & 57.50 & 55.76 \\
\model{Hala-9B} & 33.33 & 73.68 & 62.00 & 52.50 & 55.38 \\
\model{Qwen2.5-7B-Instruct} & 25.00 & \textbf{76.32} & 65.60 & 47.50 & 53.60 \\
\model{Falcon-H1-7B-Instruct} & 29.17 & 68.42 & 60.40 & 47.50 & 51.37 \\
\model{jais-adapted-13b-chat} & 33.33 & 61.84 & 64.80 & 42.50 & 50.62 \\
\model{Jais 2 8B (ours)} & 25.00 & 65.79 & 62.40 & 42.50 & 48.92 \\
\model{aya-expanse-8b} & 12.50 & 47.37 & 63.20 & 65.00 & 47.02 \\
\model{Qwen3-8B} & 25.00 & 48.68 & 69.20 & 45.00 & 46.97 \\
\model{jais-family-13b-chat} & 12.50 & 61.84 & 50.80 & 52.50 & 44.41 \\
\model{gemma-3-4b-it} & 33.33 & 59.21 & 23.60 & 60.00 & 44.04 \\
\model{c4ai-command-r7b-arabic-02-2025} & 25.00 & 63.16 & 52.40 & 35.00 & 43.89 \\
\model{jais-adapted-7b-chat} & 33.33 & 51.32 & 37.60 & 27.50 & 37.44 \\
\model{jais-family-6p7b-chat} & 16.67 & 39.47 & 20.80 & 47.50 & 31.11 \\


\midrule
\textbf{Open models $>$ 13B parameters} \\
\midrule
\model{Falcon-H1-34B-Instruct} & 33.33 & \textbf{76.32} & 71.20 & \textbf{60.00} & \textbf{60.21} \\
\model{Jais 2 70B (ours)} & \textbf{37.50} & 68.42 & \textbf{76.80} & 42.50 & 56.31 \\
\model{Gemma3-27B} & 33.33 & 71.05 & 65.60 & 55.00 & 56.25 \\
\model{Llama-3.3-70B-Instruct} & 29.17 & 75.00 & 72.80 & 42.50 & 54.87 \\
\model{Qwen2.5-72B-Instruct} & 25.00 & \textbf{76.32} & 65.60 & 47.50 & 53.60 \\
\model{Qwen2.5-32B} & 16.67 & 72.37 & 66.80 & 47.50 & 50.83 \\
\model{Llama-3.1-70B-Instruct} & 20.83 & \textbf{76.32} & 59.20 & 45.00 & 50.34 \\
\model{jais-family-30b-8k-chat} & 20.83 & 75.00 & 48.40 & 50.00 & 48.56 \\
\model{jais-adapted-70b-chat} & 29.17 & 61.84 & 60.00 & 40.00 & 47.75 \\
\model{jais-family-30b-16k-chat} & 16.67 & 68.42 & 62.80 & 42.50 & 47.60 \\
\model{gpt-oss-20b} & 20.83 & 28.95 & 0.80 & 20.00 & 17.65 \\

\bottomrule
\end{tabular}
}
\caption{\textbf{Arabic financial question--answering.} Shown is accuracy (in \%) across four multiple-choice question--answering tasks: Accounting, Business, Fatwa reasoning, and Financial Sentiment.}
\label{tab:financial-mcq}
\end{table*}

==> Tables/models_for_comparison.tex <==
\begin{table}[h]
\centering
\scriptsize
\begin{tabular}{ll}
\toprule
\textbf{Model Name} & \textbf{URL} \\
\midrule
\model{AceGPT-v2-8B-Chat} & \url{https://huggingface.co/FreedomIntelligence/AceGPT-v2-8B-Chat} \\
\model{ALLaM-7B-Instruct-preview} & \url{https://huggingface.co/humain-ai/ALLaM-7B-Instruct-preview} \\
\model{aya-23-8B} & \url{https://huggingface.co/CohereLabs/aya-23-8B} \\
\model{aya-expanse-8b} & \url{https://huggingface.co/CohereLabs/aya-expanse-8b} \\
\model{c4ai-command-r7b-arabic-02-2025} & \url{https://huggingface.co/CohereForAI/c4ai-command-r7b-arabic-02-2025} \\
\model{Falcon-H1-34B-Instruct} & \url{https://huggingface.co/tiiuae/Falcon-H1-34B-Instruct} \\
\model{Falcon-H1-7B-Instruct} & \url{https://huggingface.co/tiiuae/Falcon-H1-7B-Instruct} \\
\model{Fanar-1-9B-Instruct} & \url{https://huggingface.co/QCRI/Fanar-1-9B-Instruct} \\
\model{gemma-2-9b-it} & \url{https://huggingface.co/google/gemma-2-9b-it} \\
\model{gemma-3-12b-it} & \url{https://huggingface.co/google/gemma-3-12b-it} \\
\model{gemma-3-4b-it} & \url{https://huggingface.co/google/gemma-3-4b-it} \\
\model{Gemma3-27B-it} & \url{https://huggingface.co/google/gemma-3-27b-it} \\
\model{gpt-oss-20b} & \url{https://huggingface.co/openai/gpt-oss-20b} \\
\model{Hala-9B} & \url{https://huggingface.co/hammh0a/Hala-9B} \\
\model{jais-adapted-13b-chat} & \url{https://huggingface.co/inceptionai/jais-adapted-13b-chat} \\
\model{jais-adapted-70b-chat} & \url{https://huggingface.co/inceptionai/jais-adapted-70b-chat} \\
\model{jais-adapted-7b-chat} & \url{https://huggingface.co/inceptionai/jais-adapted-7b-chat} \\
\model{jais-family-13b-chat} & \url{https://huggingface.co/inceptionai/jais-family-13b-chat} \\
\model{jais-family-30b-16k-chat} & \url{https://huggingface.co/inceptionai/jais-family-30b-16k-chat} \\
\model{jais-family-30b-8k-chat} & \url{https://huggingface.co/inceptionai/jais-family-30b-8k-chat} \\
\model{jais-family-6p7b-chat} & \url{https://huggingface.co/inceptionai/jais-family-6p7b-chat} \\
\model{Llama-3.1-70B-Instruct} & \url{https://huggingface.co/meta-llama/Llama-3.1-70B-Instruct} \\
\model{Llama-3.1-8B-Instruct} & \url{https://huggingface.co/meta-llama/Llama-3.1-8B-Instruct} \\
\model{Llama-3.3-70B-Instruct} & \url{https://huggingface.co/meta-llama/Llama-3.3-70B-Instruct} \\
\model{Qwen2.5-32B-Instruct} & \url{https://huggingface.co/Qwen/Qwen2.5-32B-Instruct} \\
\model{Qwen2.5-72B-Instruct} & \url{https://huggingface.co/Qwen/Qwen2.5-72B-Instruct} \\
\model{Qwen2.5-7B-Instruct} & \url{https://huggingface.co/Qwen/Qwen2.5-7B-Instruct} \\
\model{Qwen3-8B} & \url{https://huggingface.co/Qwen/Qwen3-8B} \\
\model{SILMA-9B-Instruct-v1.0} & \url{https://huggingface.co/silma-ai/SILMA-9B-Instruct-v1.0} \\
\model{Yehia-7B-preview} & \url{https://huggingface.co/Navid-AI/Yehia-7B-preview} \\
\bottomrule
\end{tabular}
\caption{Models used in our experiments along with their HuggingFace repositories.}
\label{tab:models_for_comparison}
\end{table}


==> Tables/poetry_analysis_examples.tex <==
\begin{tcolorbox}[
    breakable,
    enhanced jigsaw,
    colback=gray!5,
    colframe=gray!30,
    boxrule=0.4pt,
    arc=2pt,
    left=6pt,
    right=6pt,
    top=6pt,
    bottom=6pt
]
\footnotesize
\ttfamily

\textbf{Question (Arabic):} \\
{\arabicfont
\RL{حلل البيت التالي من الناحية البلاغية: كل السيوف قواطع إن جردت وحسام لحظك قاطع في غمده}\\
}\\

\vspace{4pt}
\textbf{Jais2 Answer:}

{\arabicfont\color{green!50!black}
\begin{RLtext}
بالتأكيد، دعنا نحلل البيت الشعري التالي من الناحية البلاغية: \\
\textbf{البيت} \\
كل السيوف قواطع إن جردت  وحسام لحظك قاطع في غمده \\
\textbf{التحليل البلاغي} \\
يتميز هذا البيت بالعديد من المحسنات البديعية والصور البلاغية التي تكسبه قوة وجمالاً. إليك تحليل مفصل: \\
\textbf{1. الاستعارة المكنية} \\
\textbf{حسام لحظك}: هذا التعبير هو استعارة مكنية بارزة. الحسام يعني السيف الحاد القاطع. هنا، يشبه الشاعر نظرة المحبوب (أو المخاطب) بالسيف الحاد، ولكنه لا يصرح بالمشبه به (النظرة) مباشرة، بل يذكر شيئًا من لوازمه أو صفاته وهو الحسام. هذا يضفي على النظرة قوة خارقة وتأثيراً مميتاً حتى وهي كامنة. \\
\textbf{في غمده}: الغمد هو الغلاف الذي يوضع فيه السيف. استخدام الغمد هنا يكمل صورة الاستعارة، ويؤكد أن قوة النظرة كامنة ومستترة، ومع ذلك فهي فعالة. \\
\textbf{2. الكناية} \\
\textbf{لحظك}: اللحظ هنا لا يعني مجرد النظرة بالعين، بل يشير إلى نظرة المحبوب أو المخاطب التي تحمل في طياتها مشاعر وعواطف. يمكن اعتبار اللحظ كناية عن الشخص نفسه أو عن تأثيره القوي على الشاعر. \\
\textbf{كل السيوف قواطع إن جردت}: هذا الجزء يمكن اعتباره كناية عن القوة الكامنة والفعالية المطلقة. هو لا يقصد بالضرورة كل سيف في الواقع، بل يستخدم كل السيوف كناية عن أقصى درجات القوة والقطع. \\
\textbf{3. الطباق} \\
\textbf{قواطع إن جردت - قاطع في غمده}: هذا هو جوهر الطباق في البيت. يوجد طباق بين حالة السيف وهو مُستل (مجرّد) وحالته وهو مُستتر (في غمده). هذا التضاد يبرز المفارقة العجيبة: السيوف العادية تحتاج إلى أن تُستل لتُظهر فعاليتها، بينما نظرة المحبوب (أو المخاطب) تكون قاطعة ومؤثرة حتى وهي كامنة ومستترة. هذا يبرز قوة النظرة وتأثيرها النفسي العميق. \\
\textbf{4. الجناس} \\
\textbf{السيوف و قواطع}: يوجد جناس ناقص (غير تام) بين السيوف و قواطع. يتشاركان في بعض الحروف (السين، الواو)، مما يخلق جرساً موسيقياً خفيفاً يعزز المعنى. \\
\textbf{إن جردت و قاطع}: يوجد أيضاً جناس ناقص بين إن جردت (بمعنى إذا تم إخراجها من غمدها) و قاطع (صفة السيف). هذا التكرار الصوتي يعزز فكرة القطع والتأثير. \\
\textbf{5. المبالغة} \\
\textbf{كل السيوف قواطع إن جردت}: هذه مبالغة مقبولة في سياق الشعر. لا يقصد الشاعر أن كل سيف في الوجود قاطع بالضرورة، بل يبالغ في وصف قوة النظرة المقابلة لها. \\
\textbf{حسام لحظك قاطع في غمده}: هذه هي المبالغة الأكثر تأثيراً. فكرة أن النظرة قاطعة حتى وهي مستترة هي مبالغة تهدف إلى إبراز شدة تأثيرها النفسي والعاطفي. \\
\textbf{6. التشبيه الضمني} \\
يقارن الشاعر ضمنياً بين السيوف العادية ونظرة المحبوب. السيوف تحتاج إلى أن تُستل لتُحدث الأثر، بينما نظرة المحبوب تحدث أثرها حتى وهي كامنة. هذا التشبيه الضمني يبرز تفوق نظرة المحبوب وتأثيرها الفريد. \\
\textbf{7. قوة التعبير وجمال التصوير} \\
البيت ينجح في رسم صورة حسية قوية. هو لا يصف مجرد نظرة، بل يشبهها بأقوى الأسلحة (السيف القاطع). \\
استخدام كل السيوف يعمم القوة، ويجعل نظرة المحبوب مثالاً مطلقاً. \\
التناقض بين حالة السيف العادية (الاستلال للقطع) وحالة النظرة (القطع وهي كامنة) يخلق مفارقة مؤثرة ومفاجئة. \\
\textbf{خلاصة} \\
هذا البيت غني بالدلالات البلاغية التي تعمل معاً لخلق تأثير قوي وجميل. الاستعارة المكنية والكناية تبرزان قوة النظرة وتأثيرها العميق. الطباق يبرز المفارقة بين السيوف العادية ونظرة المحبوب. الجناس والتشبيه الضمني يعززان المعنى ويضيفان إلى جمال التعبير. بشكل عام، البيت يصور نظرة المحبوب كقوة خارقة لا تحتاج إلى إظهار صريح لتُحدث تأثيرها، بل هي مؤثرة حتى وهي كامنة، مما يعكس عمق الانبهار وقوة التأثير النفسي. \\
\end{RLtext}
}
\end{tcolorbox}


\begin{tcolorbox}[
    breakable,
    enhanced jigsaw,
    colback=gray!5,
    colframe=gray!30,
    boxrule=0.4pt,
    arc=2pt,
    left=6pt,
    right=6pt,
    top=6pt,
    bottom=6pt
]
\footnotesize
\ttfamily

\textbf{Question (Arabic):} \\
{\arabicfont
\RL{ما هو التحليل البلاغي للبيت  فَغُضَّ الطَرفَ إِنَّكَ مِن نُمَيرٍ  فَلا كَعباً بَلَغتَ وَلا كِلابا}\\
}\\

\vspace{4pt}
\textbf{Jais2 Answer:}
{\arabicfont\color{green!50!black}
\begin{RLtext}
بالتأكيد، دعنا نحلل هذا البيت من الناحية البلاغية:\\
\textbf{التحليل البلاغي}:\\

\RL{\textbf{1.  الأمر}}:\\
\RL{\textbf{فَغُضَّ الطَرفَ}:\\هذا أسلوب أمر مباشر. غضّ الطرف يعني خفض العين أو إطراقها، وغالباً ما يُستخدم للدلالة على التواضع أو الانكسار أو عدم القدرة على النظر إلى شيء أسمى. هنا، يُأمر الشاعر المخاطب بأن يُخفض طرفه، مما يوحي بأن مكانته أو قبيلته أدنى من أن تُرفع لها العين.}\\
\textbf{2.  التعليل أو الاستئناف البياني}:\\
\textbf{2إِنَّكَ مِن نُمَيرٍ}:\\هذه جملة تعليلية لما قبلها. الشاعر لا يكتفي بالأمر، بل يُبيّن سبب هذا الأمر. الانتماء إلى قبيلة نمير هو السبب الذي يُوجِب عليه غضّ الطرف. هذا يُستخدم لتأكيد المعنى وإضفاء سبب وجيه للأمر.\\
\textbf{3.  النفي}:\\
\textbf{فَلا كَعباً بَلَغتَ وَلا كِلابا}:\\هذا هو الجزء الأهم في البيت من الناحية البلاغية، وهو نفي قاطع ومُحقّر.\\
\textbf{فلا كعباً بلغتَ}:\\كعب هنا تشير إلى قبيلة بني كعب بن ربيعة. الشاعر ينفي أن يكون المخاطب قد وصل إلى مكانة قبيلة بني كعب أو شرفها.\\
\textbf{ولا كلاباً}:\\كلاب هنا تشير إلى قبيلة بني كلاب بن عامر. الشاعر ينفي أيضاً أن يكون المخاطب قد وصل إلى مكانة قبيلة بني كلاب أو شرفها.\\
\textbf{4.  المقارنة الضمنية  والتحقير}:\\
 يضع الشاعر قبيلة نمير (قبيلة المخاطب) في مقابل قبيلتي كعب وكلاب. هاتان القبيلتان (كعب وكلاب) كانتا تُعدان من القبائل ذات المكانة والقوة في العصر الجاهلي وصدر الإسلام. الانتماء إليهما كان يُعدّ مفخرة.\\
من خلال هذا النفي المزدوج، يُحقّر الفرزدق قبيلة نمير بشكل قاطع. هو يقول للمخاطب: أنت لست من قبيلة مرموقة مثل كعب أو كلاب، بل أنت من نمير، وهي قبيلة أقل شأناً.\\
\textbf{5.  البيت كشاهد على الهجاء القبلي}:\\
 يُعد هذا البيت مثالاً كلاسيكياً على الهجاء القبلي في الشعر العربي. الهدف هو إهانة المخاطب وقبيلته من خلال مقارنتهم بقبائل أخرى يُنظر إليها على أنها أدنى أو أقل شأناً.\\
 يستخدم الشاعر معرفته بالأنساب والقبائل لتعزيز قوة هجائه.\\
\textbf{خلاصة}:\\
البيت يستخدم أسلوب الأمر المُعلّل بالنسب القبلي، متبوعاً بنفي قاطع يُقارن بين قبيلة المخاطب (نمير) وقبائل أخرى (كعب وكلاب) ليُظهر تفوق الأخيرة على الأولى. هذا التركيب البلاغي يُحقّر المخاطب وقبيلته بشكل فعال، ويُبرز قوة الهجاء القبلي في الشعر العربي القديم.
\end{RLtext}
}
\end{tcolorbox}


\begin{tcolorbox}[
    breakable,
    enhanced jigsaw,
    colback=gray!5,
    colframe=gray!30,
    boxrule=0.4pt,
    arc=2pt,
    left=6pt,
    right=6pt,
    top=6pt,
    bottom=6pt
]
\footnotesize
\ttfamily

\textbf{Question (Arabic)}
{\arabicfont
\RL{ما هو التحليل البلاغي للبيت: سَلي الرِماحَ العَوالي عَن مَعالينا  وَاِستَشهِدي البيضَ هَل خابَ الرَجا فينا}\\
}

\vspace{4pt}
\textbf{Jais2 Answer}
{\arabicfont\color{green!50!black}
\begin{RLtext}
بالتأكيد، دعنا نحلل هذا البيت من الناحية البلاغية: \\
\textbf{التحليل البلاغي:1.  الاستعارة المكنية}:\\
\textbf{1.  الاستعارة المكنية}:\\
\textbf{سَلي الرِماحَ العَوالي}:\\هنا استعارة مكنية رائعة. الشاعر يُخاطب الرِماح (الرماح الطويلة) وكأنها كائن حي له لسان وعقل يُمكنه الإجابة. هو يُشخص الجماد ويُنسب إليه القدرة على السؤال عن أمجادهم. هذا يضفي على الرِماح صفة الشاهد الحي على تاريخهم وبطولاتهم. \\
\textbf{اِستَشهِدي البيضَ}:\\ مشابهة للاستعارة الأولى، حيث يُخاطب السيوف البيضاء (أو السيوف بشكل عام) ويطلب منها الشهادة. السيوف هنا أيضاً تُصبح شاهداً على أفعالهم ونصرهم. \\
\textbf{2.  التشخيص}:\\
التشخيص هو منح صفات الكائنات الحية لغيرها من الجمادات أو المعاني. في هذا البيت، الرِماح والسيوف تُعامل ككائنات حية قادرة على السؤال والشهادة. هذا يجعل هذه الأدوات الحربية أكثر قوة وتأثيراً في إيصال رسالة الشاعر. \\
\textbf{3.  الاستفهام البلاغي}:\\
\textbf{عَن مَعالينا}:\\هذا جزء من جملة سَلي الرِماحَ العَوالي عن مَعالينا. السؤال هنا ليس لطلب معلومة، بل هو لغرض بلاغي وهو التأكيد على أن الرِماح والسيوف هي أفضل من يُجيب عن أمجادهم وبطولاتهم، لأنها أدواتهم في تحقيقها. \\
\textbf{هَل خابَ الرَجا فينا}:\\هذا استفهام بلاغي آخر. هو يُؤكد على أن من رجا فيهم لم يخب رجاؤه أبداً. صيغة الاستفهام هنا تُستخدم لتقرير الحقيقة وتأكيدها بشكل أقوى من الإخبار المباشر. \\
\textbf{4.  التضاد والتوضيح}:\\
البيت يُقدم فكرة واضحة: أفعالنا وبطولاتنا (الممثلة بالرِماح والسيوف) هي التي تتحدث عنا وتُثبت مجدنا. هذا يُقابل بين الكلام العادي والفعل البطولي. \\
يُوضح الشاعر أن الرِماح والسيوف ليست مجرد أدوات قتال، بل هي سجلات حية لتاريخهم المجيد. \\
\textbf{5.  القوة التعبيرية والتصوير الحي }:\\
 البيت يرسم صورة حية وقوية للمعركة. الشاعر لا يُصف المعركة بشكل مباشر، بل يُحيل إلى أدواتها الرئيسية ليُخبر عن شدة القتال، وكثرة الأعداء الذين واجهوهم، وانتصاراتهم المتتالية. \\
استخدام الرِماح العَوالي (الطويلة) والسيوف البيض يُبرز طبيعة السلاح المستخدم ويُضفي عليها صفة القوة والوضوح (السيوف البيضاء كرمز للنصر والوضوح) \\
\textbf{6.  الفخر والاعتزاز}:\\
البيت بأكمله يُعدّ تعبيراً عن الفخر الشديد. الشاعر يُفاخر ببطولات قومه، ويُشير إلى أنهم مصدر فخر لمن يرجوهم. \\
النفي الضمني في الشطر الثاني (لم يخب الرجا فينا) يُؤكد على الثقة بالنفس والوفاء بالعهود. \\
\textbf{خلاصة}:\\
البيت يُعدّ تحفة بلاغية في الفخر والحماسة. من خلال الاستعارة المكنية والتشخيص، يُحوّل الشاعر أدوات الحرب (الرِماح والسيوف) إلى شهود أحياء على مجد قبيلته. الاستفهامات البلاغية تُعزز هذا المعنى وتُقرر الحقيقة بشكل قاطع. البيت يُبرز قوة الفعل البطولي كمصدر للمجد، ويُظهر ثقة الشاعر وقومه بأنفسهم وبأنهم لم يخذلوا أحداً.
\end{RLtext}
}
\end{tcolorbox}

==> Tables/poetry_analysis_results_sample.tex <==
\begin{table}[!ht]
\centering
\scriptsize
\setlength{\tabcolsep}{5pt}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{lrrrrr}
\toprule
\textbf{Model} &
\makecell[c]{\textbf{Poem\_\_}\\\textbf{meter}} &
\makecell[c]{\textbf{Poem\_\_}\\\textbf{genre}} &
\makecell[c]{\textbf{Poem\_\_}\\\textbf{Era}} &
\makecell[c]{\textbf{Poem\_\_}\\\textbf{Poet}} &
\makecell[c]{\textbf{Poet\_\_}\\\textbf{Era}} \\
\midrule
\multicolumn{6}{l}{\textbf{Open models $\leq$ 13B parameters}} \\
\midrule
\model{ALLaM-7B-Instruct-preview}  & 50.34 & 66.91 & 38.87 & 53.26 & 72.06 \\
\model{Falcon-H1-7B-Instruct}  & 30.07 & 56.18 & 35.27 & 49.04 & 51.05 \\
\model{Fanar-1-9B-Instruct}  & 54.63 & 72.73 & 46.39 & \textbf{60.27} & 66.81 \\
\model{Hala-9B}  & 39.60 & 69.64 & 37.77 & 52.88 & 64.50 \\
\model{SILMA-9B-Instruct-v1.0 }  & 25.64 & 63.82 & 28.99 & 36.08 & 56.30 \\
\model{Yehia-7B}  & 40.40 & 62.36 & \textbf{47.18} & 48.37 & 75.84 \\
\model{Llama-3.1-8B-Instruct}  & 22.42 & 41.64 & 27.59 & 37.14 & 40.97 \\
\model{Qwen2.5-7B-Instruct}  & 28.05 & 64.36 & 36.36 & 43.28 & 55.04 \\
\model{aya-23-8B}  & 37.05 & 57.27 & 28.37 & 43.38 & 44.12 \\
\model{aya-expanse-8b}  & 52.08 & 65.82 & 39.18 & 48.94 & 59.24 \\
\model{c4ai-command-r7b-arabic-02-2025} & 43.09 & 67.64 & 30.25 & 34.74 & 53.78 \\
\model{gemma-2-9b-it}  & 31.14 & 69.09 & 37.30 & 39.54 & 61.13 \\
\model{gemma-3-4b-it}  & 28.32 & 54.36 & 33.54 & 25.72 & 41.18 \\
\model{gemma-3-12b-it}  & 39.19 & 73.45 & 35.58 & 35.03 & 64.71 \\
\model{AceGPT-v2-8B-Chat} & 29.93 & 64.18 & 31.35 & 43.09 & 67.65 \\
\model{jais-adapted-7b-chat}  & 19.19 & 26.73 & 16.61 & 20.25 & 27.94 \\
\model{jais-family-6p7b-chat}  & 19.60 & 37.09 & 27.12 & 40.21 & 42.23 \\
\model{jais-adapted-13b-chat}  & 23.36 & 42.91 & 20.06 & 31.09 & 48.11 \\
\model{jais-family-13b-chat}  & 26.98 & 44.55 & 23.82 & 46.16 & 55.04 \\
\model{Jais-2-8B} &  \textbf{55.84} & 72.18 & 33.39 & 57.29 & \textbf{76.26} \\
\midrule
\multicolumn{6}{l}{\textbf{Open models $>$ 13B parameters}} \\
\midrule
\model{Jais-2-70B}  & \textbf{55.97} & \textbf{76.55} & 41.69 & \textbf{79.75} & \textbf{84.45} \\
\model{Llama-3.1-70B-Instruct}  & 42.68 & 75.45 & 37.62 & 47.22 & 69.12 \\
\model{Llama-3.3-70B-Instruct}  & 47.38 & 75.45 & 39.34 & 54.51 & 66.39 \\
\model{Qwen2.5-72B-Instruct}  & 51.68 & 73.82 & \textbf{46.39} & 60.65 & 72.06 \\
\model{jais-adapted-70b-chat}  & 37.05 & 65.64 & 40.44 & 46.26 & 70.80 \\
\model{Qwen2.5-32B-Instruct}  & 38.39 & 71.27 & 41.85 & 50.58 & 66.39 \\
\model{gemma-3-27b-it}  & 51.14 & \textbf{78.91} & 42.63 & 50.77 & 65.13 \\
\model{jais-family-30b-8k-chat}  & 32.48 & 49.64 & 30.88 & 46.55 & 63.87 \\
\model{jais-family-30b-16k-chat}  & 33.29 & 56.00 & 29.47 & 40.69 & 64.08 \\
\model{Falcon-H1-34B-Instruct}  & 51.14 & 71.09 & 45.30 & 51.06 & 72.27 \\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{Model accuracy on selected Arabic Poetry Analysis tasks (higher is better). 
Each column represents a prediction task of the form \textit{X\_\_Y}. 
Values are percentages.}
\label{tab:poetry_analysis_results_subset}
\end{table}

==> Tables/translation-examples.tex <==
\begin{table*}[H]
\centering
\renewcommand{\arraystretch}{1.5}
\setlength{\tabcolsep}{8pt}
\begin{tabular}{c p{0.30\textwidth} p{0.50\textwidth}}
\toprule
\textbf\scriptsize{Source - Target} & \textbf\scriptsize{Source} & \textbf\scriptsize{Target} \\
\midrule
\scriptsize{English - MSA}
&
\scriptsize\textit{One of milk's strongest selling points is the fact that it's rich in calcium. Indeed, this dairy drink does contain a decent amount of calcium, but how does it compare with other dietary sources, really? It turns out there are quite a few alternatives when it comes to foods rich in this mineral, and many actually pack higher quantities of it when compared to milk!}
&
\scriptsize{\begin{RLtext}\RL{أحد أقوى نقاط بيع الحليب هو حقيقة أنه غني بالكالسيوم. نعم، هذا المشروب الحليبي يحتوي بالفعل على كمية جيدة من الكالسيوم، ولكن كيف يقارن حقًا بمصادر الغذاء الأخرى؟ اتضح أن هناك العديد من البدائل عندما يتعلق الأمر بالأطعمة الغنية بهذا المعدن، والعديد منها يحتوي في الواقع على كميات أعلى منه مقارنة بالحليب!.}\end{RLtext}}\\
\midrule
\scriptsize{English - Moroccan} &
\scriptsize\textit{This legume is packed with protein, fiber, and, of course, calcium. One and a half cup of chickpeas contains 350 mg of calcium, which is more than a glass of milk.}
&
\scriptsize{\begin{RLtext}\RL{هاد القطاني معامر بالبروتين، الألياف، و، بطبيعة الحال، الكالسيوم. واحد الكاس ونص نتاع الحمص فيه 350 مغرام ديال الكالسيوم، لي هو كتر من كاس دالحليب.}\end{RLtext}}\\
\midrule
\scriptsize{English - Egyptian}
&
\scriptsize\textit{Yogurt is a dairy product, and as such it also contains a fair amount of calcium. We’re talking about 311 mg per cup, which is superior to a glass of milk, which contains around 305 mg.}
&
\scriptsize{\begin{RLtext}\RL{الزبادي هو منتج ألبان، و عشان كده هو كمان فيه نسبة كويسة من الكالسيوم. بنتكلم عن حوالي 311 ملغ في الكوب، وده أعلى من كوب اللبن اللي فيه حوالي 305 ملغ.}\end{RLtext}}\\
\midrule
\scriptsize{English - Algerian}
&
\scriptsize\textit{High calcium content has always been one of milk’s strongest selling points. But how much calcium is in a glass of milk, really? This will depend on how big the glass is, of course.There is about 305 mg of calcium in one cup (245 ml) of milk.}
&
\scriptsize{\begin{RLtext}\RL{المحتوى العالي من الكالسيوم كان دايماً واحد من أقوى نقاط البيع تاع الحليب. ولكن شحال من كالسيوم كاين في كاس حليب، بالصح؟ هذا يعتمد على شحال كبير الكاس، بالطبع. كاين حوالي 305 ملغ من الكالسيوم في كاس واحد (245 مل) من الحليب.}\end{RLtext}}\\
\midrule
\scriptsize{English - Tunisian}
&
\scriptsize\textit{Potatoes are a culinary staple that are used the world over to make some of the most comforting and tasty dishes you can think of. Whether you enjoy your spuds classic or with a creative twist, we think there’s something you’ll want to dig into in these 25 delicious recipes.}
&
\scriptsize{\begin{RLtext}\RL{البطاطا هي مكون أساسي في الطبخ يتستعمل في العالم الكل باش تحضرو بيه شوية من أحلى و أريح الماكلة إلي تتصورها. سوا تحب البطاطا متاعك تقليدية ولا بلمسة جديدة، نحنا نتوقّعو إنو فما حاجة تعجبك في الـ25 وصفة بنينة هاذم.}\end{RLtext}}\\
\midrule
\scriptsize{English - Levantine}
&
\scriptsize\textit{What makes a perfect baked potato? A crispy outside and a fluffy, buttery inside. Follow these directions for easy prep and baking, then top with sour cream, cheese, chives or whatever pleases your potato-loving heart.}
&
\scriptsize{\begin{RLtext}\RL{شو اللي بخلي البطاطا المشوية مثالية؟ قشرة مقرمشة ولب طري ودسم. اتبع هاي التعليمات للتحضير والخبز السهل، وبعدين حط عليها قشطة حامضة، جبنة، ثوم أخضر أو أي اشي بريح قلبك اللي بحب البطاطا.}\end{RLtext}}\\
\midrule
\scriptsize{English - Saudi}
&
\scriptsize\textit{Dried figs are very good. They are rich in fiber, potassium, and antioxidants called polyphenols. They are very good for the digestive system and can help as a mild natural laxative.}
&
\scriptsize{\begin{RLtext}\RL{التين المجفف ترى مرة زين. غني بالألياف والبوتاسيوم ومضادات الأكسدة اللي يسمونها البوليفينول. مرة زين للجهاز الهضمي وممكن يساعد كملين طبيعي خفيف.}\end{RLtext}}\\
\bottomrule
\end{tabular}
\caption{Translation examples.}
\label{tab:translation_examples_new}
\end{table*}

==> Tables/translation_results.tex <==
\begin{table*}[htb]
\centering
\scriptsize
\setlength{\tabcolsep}{1.5pt}
\resizebox{0.8\textwidth}{!}{%
\begin{tabular}{
  l *{9}{r} 
}
\toprule
\multirow{2}{*}{\textbf{Model}} &
\multicolumn{3}{c}{\textbf{ATHAR}} &
\multicolumn{3}{c}{\textbf{Arab-Acquis}} &
\multicolumn{3}{c}{\textbf{ArzEn-ST}} \\
\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}
& \multicolumn{1}{c}{art$\to$en} & \multicolumn{1}{c}{en$\to$art} & \multicolumn{1}{c}{Avg}
& \multicolumn{1}{c}{ar$\to$en} & \multicolumn{1}{c}{en$\to$ar} & \multicolumn{1}{c}{Avg}
& \multicolumn{1}{c}{arz$\to$en} & \multicolumn{1}{c}{en$\to$arz} & \multicolumn{1}{c}{Avg} \\
\midrule
\scriptsize
\textbf{Open models $\leq$ 13B parameters} \\
\midrule
\model{Jais-2-8B} & \bf 21.82 & \bf 12.79 & \bf 17.31 & \bf 56.97 & \bf 32.58 & \bf 44.78 & \bf 30.10 & \bf 15.39 & \bf 22.75 \\
\model{c4ai-command-r7b-12-2024} & 12.46 & 3.22 & 7.84 & 49.58 & 25.52 & 37.55 & 27.51 & 7.56 & 17.54 \\
\model{Falcon-H1-7B-Instruct} & 13.10 & 2.10 & 7.60 & 48.10 & 17.4& 32.75& 24.70 & 5.50 & 15.10 \\
\model{ALLaM-7B-Instruct-preview-v1} & 10.84 & 1.58 & 6.21 & 29.94 & 17.01 & 23.48 & 20.52 & 8.63 & 14.58 \\
\model{SILMA-9B-Instruct-v1.0} & 11.23 & 2.94 & 7.09 & 38.40 & 20.20 & 29.30 & 20.23 & 6.32 & 13.28 \\
\model{Yehia-7B} & 11.84 & 2.94 & 7.39 & 39.66 & 29.31 & 34.49 & 24.14 & 8.67 & 16.41 \\
\model{jais-adapted-13b-chat} & 9.82 & 1.95 & 5.89 & 34.35 & 26.47 & 30.41 & 23.54 & 5.82 & 14.68\\
\model{aya-23-8B} & 10.39 & 2.24 & 6.32 & 46.69 & 26.17 & 36.43 & 21.11 & 4.99 & 13.05 \\
\model{Qwen3-8B} & 11.73 & 1.95 & 6.84 & 40.64 & 21.09 & 30.86 & 20.18 & 3.78 & 11.98 \\
\model{jais-adapted-7b-chat} & 6.23 & 0.27 & 3.25 & 32.00 & 14.51 & 23.25 & 12.63 & 3.91 & 8.27\\
\model{aya-expanse-8b} & 9.04 & 2.79 & 5.92 & 36.70 & 25.69 & 31.20 & 10.99 & 4.00 & 7.50 \\
\model{Qwen2.5-7B-Instruct} & 5.65 & 0.88 & 3.27 & 28.89 & 13.80 & 21.35 & 8.92 & 2.58 & 5.75 \\
\model{Fanar-1-9B-Instruct} & 5.92 & 1.65 & 3.79 & 31.69 & 21.89 & 26.79 & 9.67 & 1.78 & 5.73 \\
\model{jais-family-6p7b-chat} & 1.93 & 0.41 & 1.17 & 6.67 & 12.02 & 9.34 & 6.83 & 3.94 & 5.38\\
\model{jais-family-13b-chat} & 5.87 & 1.79 & 3.83 & 21.44 & 18.62 & 20.03 & 13.30 & 3.61 & 8.46\\
\model{gemma-2-9b-it} & 7.67 & 0.24 & 3.96 & 37.46 & 4.88 & 21.17 & 7.93 & 1.12 & 4.53 \\
\model{Llama-3.1-8B-Instruct} & 4.13 & 0.46 & 2.30 & 21.70 & 17.97 & 19.84 & 5.80 & 0.99 & 3.40 \\
\model{gemma-3-12b-it} & 2.71 & 0.13 & 1.42 & 9.37 & 4.12 & 6.75 & 3.39 & 0.83 & 2.11 \\
\model{gemma-3-4b-it} & 2.13 & 0.27 & 1.20 & 7.22 & 3.29 & 5.26 & 2.87 & 0.71 & 1.79 \\
\model{AceGPT-7B-chat} & 1.88 & 0.25 & 1.07 & 10.72 & 2.00 & 6.36 & 2.74 & 0.66 & 1.70 \\
\model{Hala-9B} & 0.34 & 0.61 & 0.48 & 2.33 & 5.92 & 4.13 & 0.36 & 0.47 & 0.42 \\

\midrule
\textbf{Open models $>$ 13B parameters} \\
\midrule
\bf \model{Jais-2-70B} & \bf 24.92 & \bf 15.06 & \bf 19.99 & \bf 60.61 & \bf 30.65 & \bf 45.63 & \bf 35.66 & \bf 17.97 & \bf 26.81 \\
\model{Falcon-H1-34B-Instruct} & 13.10 & 2.10 & 7.60 & 48.10 & 17.40 & 32.75 & 24.70 & 5.50 & 15.10\\
\model{Llama-3.3-70B-Instruct} & 13.72 & 0.99 & 7.36 & 53.45 & 26.59 & 40.02 & 26.83 & 1.34 & 14.09 \\
\model{Llama-3.1-70B-Instruct} & 9.93 & 2.13 & 6.03 & 53.93 & 27.01 & 40.47 & 21.89 & 4.60 & 13.25 \\
\model{Qwen2.5-72B-Instruct} & 11.68 & 2.38 & 7.03 & 49.84 & 25.28 & 37.56 & 15.84 & 7.17 & 11.51 \\
\model{jais-family-30b-8k-chat} & 8.49 & 2.06 & 5.27 & 22.77 & 18.85 & 20.81 & 14.02 & 4.82 & 9.42\\
\model{Qwen2.5-32B-Instruct} & 9.00 & 1.39 & 5.20 & 37.34 & 13.50 & 25.42 & 15.80 & 2.38 & 9.09 \\
\model{jais-adapted-70b-chat} \ttodo{MISSING}\\
\model{jais-family-30b-16k-chat} & 9.24 & 1.85 & 5.54 & 31.06 & 19.00 & 25.03 & 19.23 & 4.76 & 7.23\\
\model{gemma3-27b-it} & 2.75 & 0.18 & 1.47 & 10.28 & 4.39 & 7.34 & 3.50 & 0.86 & 2.18 \\
\model{gpt-oss-20b} & 1.67 & 0.20 & 0.94 & 6.27 & 3.39 & 4.83 & 3.25 & 0.69 & 1.97\\
\midrule
\textbf{Closed models} \\
\midrule
\model{Gemini-2.5-pro} & 17.38 & 1.97 & 9.68 & 62.74 & 30.64 & 46.69 & 26.19 & 13.22 & 19.71 \\
\model{Gemini-2.5-flash} & 14.81 & 2.74 & 8.78 & 58.80 & 32.42 & 45.61 & 29.42 & 13.89 & 21.66 \\
\model{GPT-5} & 15.20 & 0.78 & 7.99 & 52.77 & 29.55 & 41.16 & 25.22 & 11.85 & 18.54 \\
\model{mistral-saba} & 14.58 & 3.46 & 9.02 & 49.66 & 30.55 & 40.11 & 24.56 & 7.35 & 15.96 \\
\bottomrule
\end{tabular}%
}
\caption{\textbf{Dialectal Arabic translation}: results for ATHAR, Arab-Acquis, and ArzEn-ST benchmarks.}
\label{tab:results_extra}
\end{table*}

% \textbf{Open models $\leq$ 13B parameters} \\
% \midrule

% \midrule
% \textbf{Open models $>$ 13B parameters} \\
% \midrule

% \midrule
% \textbf{Closed models} \\
% \midrule


\begin{table*}[!t]
\centering
\small
\setlength{\tabcolsep}{1.4pt}
\resizebox{\textwidth}{!}{
\begin{tabular}{
  l *{13}{r} 
}
\toprule
\multirow{2}{*}{\textbf{Model}} &
\multicolumn{5}{c}{\textbf{Sadid}} &
\multicolumn{3}{c}{\textbf{Tarjama-25}} &
\multicolumn{5}{c}{\textbf{WMT24++}} \\
\cmidrule(lr){2-6}\cmidrule(lr){7-9}\cmidrule(lr){10-14}
& \multicolumn{1}{c}{{apc$\to$en}} & \multicolumn{1}{c}{arz$\to$en} & \multicolumn{1}{c}{en$\to$apc} & \multicolumn{1}{c}{en$\to$arz} & \multicolumn{1}{c}{Avg}
& \multicolumn{1}{c}{ar$\to$en} & \multicolumn{1}{c}{en$\to$ar} & \multicolumn{1}{c}{Avg}
& \multicolumn{1}{c}{ars$\to$en} & \multicolumn{1}{c}{arz$\to$en} & \multicolumn{1}{c}{en$\to$ars} & \multicolumn{1}{c}{en$\to$arz} & \multicolumn{1}{c}{Avg} \\
\midrule
\textbf{Open models $\leq$ 13B parameters} \\
\midrule
\model{Jais-2-8B}& 20.21 & 37.00 & 12.15 & 13.82 & 20.8 & 42.37 & 29.76 & 36.07 & 13.92 & 15.10 & 3.05 & 13.09 & 11.51 \\
\model{ALLaM-7B-Instruct-preview-v1}& 23.21 & 22.16 & 12.00 & 16.17 & 18.39 & 45.66 & 33.12 & 39.39 & 16.59 & 15.34 & 7.29 & 8.88 & 12.03 \\
\model{Falcon-H1-7B-Instruct} & 30.43 & 30.81 & 6.22 & 7.54 & 18.75 &\ttodo{MISSING} & & & 17.56 & 16.82 & 4.66 & 5.08 & 11.03\\
\model{Fanar-1-9B-Instruct} & 9.56 & 9.63 & 1.74 & 2.49 & 5.86 & 41.01 & 34.24 & 37.63 & 9.74 & 10.56 & 3.17 & 3.37 & 6.71 \\
\model{Hala-9B}& 0.23 & 0.21 & 0.71 & 0.78 & 0.48 & 1.48 & 28.04 & 14.76 & 0.50 & 0.50 & 2.01 & 1.39 & 1.10 \\
\model{SILMA-9B-Instruct-v1.0 } & 34.69 & 33.33 & 9.56 & 10.76 & 22.09 & 41.12 & 21.42 & 31.27 & 20.56 & 18.67 & 7.37 & 6.45 & 13.26 \\
\model{Yehia-7B} & 35.51 & 33.67 & 12.24 & 14.85 & 24.07 & 45.37 & 40.78 & 43.08 & 18.83 & 18.19 & 8.43 & 10.91 & 14.09 \\
\model{Llama-3.1-8B-Instruct} & 10.59 & 9.69 & 0.65 & 1.24 & 5.54 & 26.33 & 25.15 & 25.74 & 6.86 & 5.75 & 1.31 & 2.01 & 3.98 \\
\model{Qwen2.5-7B-Instruct} & 10.09 & 10.88 & 1.98 & 3.89 & 6.71 & 39.44 & 20.97 & 30.21 & 8.92 & 9.75 & 3.60 & 3.76 & 6.51 \\
\model{aya-23-8B} & 31.02 & 29.39 & 10.50 & 11.64 & 20.64 & 37.79 & 34.03 & 35.91 & 18.87 & 17.53 & 8.25 & 6.06 & 12.68 \\
\model{aya-expanse-8b} & 11.43 & 14.99 & 9.36 & 10.65 & 11.61 & 41.47 & 33.86 & 37.67 & 12.70 & 13.77 & 7.66 & 5.27 & 9.85 \\
\model{gemma-2-9b-it} & 9.41 & 10.58 & 0.76 & 0.92 & 5.42 & 40.88 & 28.30 & 34.59 & 8.53 & 11.25 & 1.55 & 1.50 & 5.71 \\
\model{gemma-3-4b-it} & 2.61 & 2.61 & 0.56 & 0.65 & 1.61 & 28.41 & 33.48 & 30.95 & 3.93 & 3.76 & 1.30 & 1.44 & 2.61 \\
\model{AceGPT-v2-8B-Chat} & 4.59 & 5.07 & 0.70 & 0.87 & 2.81 & 47.54 & 31.25 & 39.4 & 6.98 & 7.01 & 1.40 & 1.24 & 4.16\\
\model{Qwen3-8B} & 28.65 & 26.11 & 7.79 & 8.88 & 17.86 & 47.54 & 31.25 & 39.40 & 6.98 & 7.01 & 1.40 & 1.24 & 4.16 \\
\model{c4ai-command-r7b-12-2024} & 37.15 & 35.12 & 10.77 & 12.74 & 23.95 & 48.49 & 38.29 & 43.39 & 21.34 & 19.90 & 8.71 & 7.07 & 14.26 \\
\model{jais-adapted-7b-chat} & 15.99 & 20.34 & 5.82 & 7.32 & 12.37 & 27.79 & 11.39 & 19.59 & 10.00 & 13.41 & 3.49 & 3.96 & 7.72\\
\model{jais-family-6p7b-chat} & 6.89 & 7.53 & 5.72 & 7.77 & 6.98 & 26.19 & 19.44 & 22.81 & 3.17 & 5.42 & 4.26 & 3.83 & 4.17\\
\model{gemma-3-12b-it} & 3.40 & 3.33 & 0.65 & 0.86 & 2.06 & 27.29 & 29.07 & 28.18 & 4.46 & 4.34 & 1.33 & 1.63 & 2.94 \\
\model{jais-adapted-13b-chat} & 34.58 & 33.65 & 10.32 & 9.47 & 22.00 & 32.33 & 16.64 & 24.49 & 18.45 & 18.02 & 7.16 & 5.94 & 12.39\\
\model{jais-family-13b-chat} & 18.60 & 18.83 & 8.69 & 9.16 & 13.82 & 25.13 & 18.18 & 21.65 & 4.41 & 6.85 & 6.09 & 4.19 & 5.38\\
\midrule
\textbf{Open models $>$ 13B parameters} \\
\midrule
\model{Jais-2-70B} & 36.29 & 30.77 & 11.34 & 13.19 & 22.90 & 51.73 & 38.80 & 45.27 & 20.29 & 20.48 & 7.76 & 13.88 & 15.61 \\
\model{Llama-3.1-70B-Instruct} & 27.83 & 28.61 & 4.62 & 7.60 & 17.17 & 51.75 & 36.40 & 44.08 & 19.01 & 17.90 & 3.48 & 5.22 & 11.40 \\
\model{Llama-3.3-70B-Instruct} & 34.61 & 34.64 & 1.03 & 1.52 & 17.95 & 47.71 & 35.22 & 41.47 & 21.20 & 20.04 & 3.74 & 1.81 & 11.19 \\
\model{Qwen2.5-32B-Instruct} & 14.66 & 16.41 & 1.92 & 3.26 & 9.06 & 44.81 & 27.62 & 36.22 & 12.10 & 13.59 & 7.08 & 3.53 & 8.24 \\
\model{Qwen2.5-72B-Instruct}& 17.76 & 20.51 & 7.19 & 8.74 & 13.55 & 50.38 & 34.71 & 42.55 & 16.54 & 16.09 & 1.10 & 7.03 & 11.69 \\
\model{gemma-3-27b -it}& 3.42 & 3.37 & 0.56 & 0.94 & 2.07 & 33.82 & 23.04 & 28.43 & 4.28 & 4.35 & 1.10 & 1.87 & 2.90 \\
\model{jais-family-30b-8k-chat} & 23.38 & 20.81 & 8.74 & 9.33 & 15.57 & 38.10 & 23.39 & 30.74 & 8.09 & 7.68 & 6.08 & 4.98 & 6.71\\
\model{jais-family-30b-16k-chat} & 34.05 & 29.76 & 8.94 & 9.67 & 20.6 & 36.78 & 25.81 & 31.29 & 14.55 & 15.86 & 6.88 & 5.35 & 10.66\\
\model{jais-adapted-70b-chat} & 10.52 & 9.91 & 11.59 & 14.30 & 11.58 & 43.31 & 34.27 & 38.79 & 5.63 & 4.84 & 8.54 & 8.21 & 6.8\\
\model{gpt-oss-20b} & 2.68 & 2.64 & 0.69 & 0.76 & 1.69 & 13.52 & 6.95 & 10.24 & 2.85 & 2.79 & 0.88 & 1.04 & 1.89\\
\midrule
\textbf{Closed models} \\
\midrule
\model{GPT-5} & 40.16 & 36.64 & 13.57 & 20.24 & 27.65 & 54.36 & 38.32 & 46.34 & 22.76 & 21.18 & 8.06 & 14.29 & 16.57 \\
\model{Gemini-2.5-pro} & 44.3 & 41.3 & 15.0 & 22.2 & 30.7 & 55.0 & 45.4 & 50.2 & 25.8 & 24.0 & 8.8 & 13.6 & 18.11\\
\model{Gemini-2.5-flash} & 43.48 & 40.62 & 15.67 & 21.47 & 30.31 & 61.32 & 51.10 & 56.21 & 24.69 & 22.98 & 10.20 & 13.63 & 17.88 \\
\model{mistral-saba} & 40.99 & 38.51 & 13.30 & 14.55 & 26.84 & \ttodo{MISSING} & & & 22.84 & 21.67 & 7.44 & 7.34 & 14.82 \\
\bottomrule
\end{tabular}}
\caption{\textbf{Dialectal Arabic translation:} results for Sadid,Tarjama-25, and WMT24++ benchmarks.}
\label{tab:translation_results_sadid_tarjama_wmt24}
\end{table*}

% \textbf{Open models $\leq$ 13B parameters} \\
% \midrule

% \midrule
% \textbf{Open models $>$ 13B parameters} \\
% \midrule

% \midrule
% \textbf{Closed models} \\
% \midrule


==> commented_text_1.tex <==
% \section{Detailed Zero-Shot Evaluation Results}

% Table \ref{tab:results:arabic_full} and Table \ref{tab:results:english_full} show the detailed zero-shot evaluation results for Arabic and English, respectively.


% \begin{table}[h!]
% \centering
% \resizebox{\linewidth}{!}{
% \begin{tabular}{lcccccccccccccccc}
%     \toprule
%      & \multicolumn{1}{c}{} & \multicolumn{4}{c}{Knowledge} && \multicolumn{6}{c}{Commonsense Reasoning}&& \multicolumn{2}{c}{Misinformation \& Bias}& \multicolumn{1}{r}{} \\
%      \cmidrule{3-6}\cmidrule{8-13}\cmidrule{15-16}
%     \multirow{-2}{*}{Models (\#size)} & \multicolumn{1}{c}{\multirow{-2}{*}{}} & \multicolumn{1}{c}{EXAMS} & \multicolumn{1}{c}{MMLU$_H$} & \multicolumn{1}{c}{MMLU$_M$}& \multicolumn{1}{c}{LitQA} && \multicolumn{1}{c}{HellaSwag} & \multicolumn{1}{c}{PIQA} & \multicolumn{1}{c}{BoolQ} & \multicolumn{1}{c}{SituatedQA} & \multicolumn{1}{c}{ARC-C} & \multicolumn{1}{c}{OBQA}  && \multicolumn{1}{c}{TruthfulQA} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}CrowS-Pairs\end{tabular}} & \multicolumn{1}{r}{\multirow{-2}{*}{Avg}} \\
%     \midrule
%     Random &  & 25.0 & 25.0 & 25.0 & 25.0 &  & 25.0 & 50.0 & 50.0 & 33.3 & 25.0 & 25.0 &  & 44.5 & 50.0 & 33.6 \\
%     \hdashline
%     AraT5 (220M) &  & 24.7 & 23.2 & 23.8 & 26.3 &  & 25.5 & 50.4 & 58.2 & 33.9 & 24.7 & 25.4 &  & 20.9 & 47.2 & 32.0 \\
%     AraT5-v2 (220M) &  & 24.4 & 24.6 & 24.7 & 25.7 &  & 25.0 & 48.9 & 59.0 & 35.5 & 23.5 & 24.8 &  & 48.1 & 50.5 & 34.6 \\
%     AraBART (550M) &  & 26.5 & 27.7 & 27.5 & 34.3 &  & 28.1 & 52.6 & 57.1 & 34.6 & 25.1 & 28.6 &  & 49.8 & 48.8 & 36.7 \\
%     BLOOM (1.1B) &  & 29.4 & 29.8 & 28.0 & 35.4 &  & 32.8 & 54.5 & 61.5 & 36.5 & 22.6 & 26.8 &  & 46.7 & 51.9 & 38.0 \\
%     BLOOMz (1.1B)* & & 31.3 & 31.1 & 28.2 & 33.1 &  & 33.6 & 55.0 & 60.4 & 39.8 & 22.8 & 27.2 &  & 47.7 & 54.7 & 38.7 \\
%     mT5-large (1.2B)* & & 27.6 & 22.4 & 22.3 & 23.1 &  & 25.9 & 52.0 & 62.2 & 35.8 & 21.0 & 25.6 &  & 50.6 & 50.5 & 35.3 \\
%     mT0-large (1.2B)* & & 23.7 & 29.2 & 27.6 & 33.1 &  & 29.1 & 52.6 & 63.0 & 38.1 & 22.0 & 26.8 &  & 48.4 & 43.4 & 36.4 \\
%     BLOOM (1.7B) &  & 31.1 & 29.0 & 27.2 & 34.9 &  & 34.3 & 55.8 & 56.8 & 36.3 & 23.9 & 27.0 &  & 44.8 & 53.1 & 37.9 \\
%     BLOOMz (1.7B)* & & 33.6 & 31.3 & 29.2 & 38.3 &  & 31.7 & 56.4 & 71.7 & 41.7 & 27.0 & 29.0 &  & 46.3 & 55.1 & 40.9 \\
%     \hdashline
%     BLOOM (3B) &  & 30.2 & 29.6 & 27.9 & 41.7 &  & 37.1 & 56.3 & 62.2 & 36.9 & 23.8 & 27.8 &  & 44.0 & 55.1 & 39.4 \\
%     BLOOMz (3B)* & & 35.1 & 31.8 & 29.8 & 38.3 &  & 33.7 & 55.7 & 75.7 & 41.1 & 27.7 & 28.4 &  & 47.5 & 55.1 & 41.7 \\
%     mT0-xl (3.7B)* & & 25.6 & 25.4 & 26.7 & 30.9 &  & 27.8 & 50.7 & 62.0 & 35.6 & 26.0 & 29.4 &  & 45.3 & 47.4 & 36.1 \\
%     mT0-xl (3.7B)* & & 27.6 & 34.6 & 29.8 & 33.7 &  & 30.7 & 54.4 & 68.1 & 41.0 & 23.1 & 29.0 &  & 42.7 & 48.7 & 38.6 \\
    
%     \hdashline
%     BLOOM (7.1B) &  & 34.0 & 30.3 & 28.2 & 37.1 &  & 40.9 & 58.4 & 59.9 & 39.1 & 27.3 & 28.0 &  & 44.4 & 53.5 & 40.1 \\
%     BLOOMz (7.1B)* & & 34.9 & 35.2 & 31.0 & 44.0 &  & 38.1 & 59.1 & 66.6 & 42.8 & 30.2 & 29.2 &  & 48.4 & 55.8 & 42.9 \\
%     LLaMA (7B) &  & 26.7 & 30.6 & 28.1 & 32.0 &  & 30.3 & 50.9 & 45.5 & 35.1 & 24.1 & 30.4 &  & 46.3 & 46.0 & 35.5 \\
%     LLaMA2 (7B)* &  & 26.7 & 30.2 & 27.8 & 31.4 &  & 32.3 & 50.0 & 63.8 & 35.6 & 25.0 & 29.0 &  & 46.7 & 48.3 & 37.2 \\
%     LLaMA2-chat (7B) &  & 25.4 & 29.7 & 28.0 & 29.7 &  & 31.5 & 51.6 & 60.9 & 35.9 & 25.2 & 28.8 &  & 48.2 & 47.2 & 36.8 \\
%     Falcon (7B) &  & 27.6 & 29.1 & 27.5 & 25.7 &  & 29.8 & 50.5 & 61.8 & 36.3 & 22.6 & 27.0 &  & 47.7 & 45.0 & 35.9 \\
%     Falcon-Instruct (7B)* & & 22.4 & 25.0 & 25.3 & 25.7 &  & 29.4 & 52.8 & 57.6 & 35.7 & 23.3 & 26.4 &  & 46.9 & 47.8 & 34.9 \\
%     \hdashline
%     mT0-xxl (13B)* & & 26.9 & 25.5 & 26.1 & 33.7 &  & 27.9 & 52.9 & 62.2 & 35.9 & 26.2 & 29.8 &  & 45.7 & 49.6 & 36.9 \\
%     mT0-xxl (13B)* & & 31.5 & 35.3 & 31.2 & 36.6 &  & 33.9 & 56.1 & 77.8 & 44.7 & 26.1 & 27.8 &  & 44.5 & 45.3 & 40.9 \\
%     LLaMA (13B) &  & 27.6 & 30.2 & 28.2 & 33.7 &  & 32.0 & 51.0 & 62.5 & 36.3 & 25.4 & 30.0 &  & 45.6 & 52.7 & 37.9 \\
%     LLaMA2 (13B) &  & 29.2 & 30.4 & 28.4 & 32.0 &  & 34.3 & 52.9 & 63.8 & 36.4 & 24.3 & 30.0 &  & 45.5 & 49.9 & 38.1 \\
%     LLaMA2-chat (13B)* & & 26.3 & 31.5 & 29.1 & 33.1 &  & 32.0 & 52.1 & 66.0 & 36.3 & 24.1 & 28.4 &  & 48.6 & 50.0 & 38.1 \\
%     \midrule
%     Our Models &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
%     \midrule
%     \modelname{} (1.3B)  &  & 37.5 & 27.8 & 27.3 & 44.0 &  & 37.1 & 60.8 & 62.1 & 36.4 & 25.5 & 27.4 &  & 44.8 & 52.4 & 40.3 \\
%     \modelnametuned{} (1.3B)* & & 34.5 & 32.5 & 29.2 & 39.4 &  & 40.1 & 58.5 & 62.5 & 39.1 & 27.0 & 29.6 &  & 47.1 & 51.9 & 41.0 \\
%     \hdashline
%     \modelname{} (6.7B)  &  & 35.9 & 30.7 & 28.8 & 50.9 &  & 47.1 & 65.1 & 63.0 & 39.3 & 29.1 & 29.6 &  & 43.3 & 55.2 & 43.2 \\
%     \modelnametuned{} (6.7B)* & & 40.9 & 37.8 & 32.1 & 47.4 &  & 52.6 & 65.6 & 69.9 & 47.1 & 35.2 & 31.6 &  & 44.3 & 52.4 & 46.4 \\
%     \hdashline
%     \modelname{} (13B)  &  & 40.4 & 31.1 & 30.0 & 58.3 &  & 57.7 & 67.6 & 62.6 & 42.5 & 35.8 & 32.4 &  & 41.1 & 58.4 & 46.5 \\
%     % \modelnametuned{} (13B)* & & 40.4 & 35.1 & 32.5 & 49.1 &  & 60.5 & 67.5 & 68.7 & 48.0 & 39.2 & 31.6 &  & 45.6 & 57.0 & 47.9 \\
%     %V3.6
%     \modelnametuned{} (13B)* & & 39.7 & 39.3 & 34.0 & 52.6 &  & 61.4 & 67.5 & 65.7 & 47.0 & 40.7 & 31.6 &  & 44.8 & 56.4 & 48.4 \\
%     \bottomrule
% \end{tabular}}
% \caption{Full results for \textbf{Arabic} (zero-shot). ``Average'' denotes the mean score computed across the entire dataset, and ``*'' indicates that the model is fine-tuned  using general instructional datasets. MMLU$_H$ and MMLU$_M$ mean that the datasets are translated by a human and by a machine, respectively.}
% \label{tab:results:arabic_full}
% \end{table}


% \begin{table}[h!]
% \centering
% \resizebox{\linewidth}{!}{
% \begin{tabular}{lccccccccccccccc}
%     \toprule
%      & \multicolumn{1}{c}{}& \multicolumn{2}{c}{Knowledge} && \multicolumn{7}{c}{Commonsense Reasoning}&& \multicolumn{2}{c}{Misinformation \& Bias}& \multicolumn{1}{r}{} \\
%      \cmidrule{3-4}\cmidrule{6-12}\cmidrule{14-15}
%     \multirow{-2}{*}{Models (\#size)} & \multicolumn{1}{c}{\multirow{-2}{*}{}} & \multicolumn{1}{c}{MMLU} & \multicolumn{1}{c}{RACE} && \multicolumn{1}{c}{HellaSwag} & \multicolumn{1}{c}{PIQA} & \multicolumn{1}{c}{BoolQ} & \multicolumn{1}{c}{SituatedQA} & \multicolumn{1}{c}{ARC-C} & \multicolumn{1}{c}{OBQA} & \multicolumn{1}{c}{Winogrande} && \multicolumn{1}{c}{TruthfulQA} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}CrowS-Pairs\end{tabular}} & \multicolumn{1}{r}{\multirow{-2}{*}{Avg}} \\
%     \midrule
%    Random &  & 25.0 & 25.0 &  & 25.0 & 50.0 & 50.0 & 33.3 & 25.0 & 25.0 & 50.0 &  & 44.5 & 50.0 & 36.6 \\
%    \hdashline
%     AraT5 (220M) &  & 24.2 & 23.7 &  & 26.0 & 49.7 & 39.0 & 35.2 & 27.0 & 26.0 & 49.6 &  & 22.4 & 51.4 & 34.0 \\
%     AraT5-v2 (220M) &  & 24.7 & 24.6 &  & 26.2 & 49.3 & 38.0 & 37.1 & 23.3 & 25.2 & 51.4 &  & 47.7 & 51.1 & 36.2 \\
%     AraBART (550M) &  & 27.5 & 24.1 &  & 28.5 & 51.5 & 42.6 & 38.8 & 22.6 & 30.6 & 50.2 &  & 46.7 & 53.8 & 37.9 \\
%     BLOOM (1.1B) &  & 28.3 & 32.6 &  & 41.8 & 67.1 & 59.1 & 43.8 & 25.7 & 29.4 & 54.9 &  & 41.8 & 62.4 & 44.3 \\
%     BLOOMz (1.1B)* & & 28.8 & 35.7 &  & 42.2 & 68.2 & 62.1 & 50.2 & 27.2 & 31.4 & 54.1 &  & 44.4 & 60.4 & 45.9 \\
%     mT5-large (1.2B) & & 23.5 & 27.7 &  & 26.8 & 51.3 & 38.7 & 38.3 & 23.1 & 31.6 & 51.5 &  & 47.8 & 51.9 & 37.5 \\
%     mT0-large (1.2B)* & & 28.5 & 32.8 &  & 31.0 & 63.1 & 68.2 & 47.3 & 22.4 & 27.2 & 51.6 &  & 42.5 & 57.9 & 43.0 \\
%     BLOOM (1.7B) &  & 27.7 & 33.2 &  & 46.6 & 70.1 & 61.8 & 44.2 & 26.8 & 30.0 & 57.1 &  & 41.3 & 64.8 & 45.8 \\
%     BLOOMz (1.7B)* & & 30.7 & 39.7 &  & 49.1 & 70.7 & 87.9 & 57.5 & 33.9 & 34.0 & 57.8 &  & 40.0 & 64.1 & 51.4 \\
%     \hdashline
%     BLOOM (3B) &  & 28.3 & 35.2 &  & 52.7 & 70.5 & 61.6 & 43.5 & 30.5 & 32.2 & 58.7 &  & 40.6 & 64.9 & 47.2 \\
%     BLOOMz (3B)* & & 32.0 & 46.0 &  & 56.6 & 74.7 & 93.3 & 62.2 & 38.4 & 38.8 & 60.6 &  & 40.3 & 62.1 & 55.0 \\
%     mT5-xl (3.7B) & & 27 & 32.9 &  & 30.9 & 55.7 & 57.4 & 40.8 & 25.8 & 33.8 & 52.6 &  & 42.8 & 49.8 & 40.9 \\
%     mT0-xl (3.7B)* & & 31.1 & 38.3 &  & 35.7 & 65.6 & 80.6 & 52.8 & 25.2 & 29.0 & 51.6 &  & 39.8 & 56.9 & 46.1 \\
%     \hdashline
%     BLOOM (7.1B) &  & 28.6 & 36.5 &  & 59.6 & 73.6 & 62.9 & 46.5 & 33.4 & 35.8 & 64.4 &  & 38.9 & 68.9 & 49.9 \\
%     BLOOMz (7.1B)* & & 33.9 & 45.6 &  & 63.1 & 77.4 & 91.7 & 59.7 & 43.6 & 42.0 & 65.3 &  & 45.2 & 65.6 & 57.6 \\
%     LLaMA (7B) &  & 29.7 & 40.0 &  & 73.0 & 77.4 & 73.1 & 43.2 & 41.4 & 42.4 & 66.9 &  & 34.1 & 55.3 & 52.4 \\
%     LLaMA2 (7B) &  & 29.9 & 40.1 &  & 73.0 & 77.0 & 71.1 & 42.7 & 40.5 & 40.8 & 67.2 &  & 39.6 & 71.1 & 53.9 \\
%     LLaMA2-chat (7B)* &  & 30.8 & 44.1 &  & 73.4 & 76.7 & 80.8 & 45.6 & 42.9 & 41.4 & 64.8 &  & 44.9 & 69.8 & 55.9 \\
%     Falcon (7B) &  & 29.4 & 37.3 &  & 76.3 & 80.5 & 73.5 & 43.2 & 43.5 & 44.4 & 67.3 &  & 34.3 & 72.4 & 54.7 \\
%     Falcon-Instruct (7B)* & & 28.0 & 37.0 &  & 69.7 & 78.5 & 70.8 & 46.5 & 42.8 & 41.0 & 66.5 &  & 44.1 & 71.2 & 54.2 \\
%     \hdashline
%     mT5-xxl (13B) & & 26.7 & 33.2 &  & 31.9 & 56.4 & 45.2 & 39.8 & 26.5 & 33.6 & 51.5 &  & 41.1 & 48.5 & 39.5 \\
%     mT0-xxl (13B)* & & 32.6 & 43.6 &  & 42.2 & 67.6 & 87.6 & 55.4 & 29.4 & 35.2 & 54.9 &  & 43.4 & 59.0 & 50.1 \\
%     LLaMA (13B) &  & 30.1 & 39.3 &  & 76.2 & 79.1 & 68.5 & 43.7 & 44.6 & 42.2 & 70.1 &  & 39.9 & 49.3 & 53.0 \\
%     LLaMA2 (13B) &  & 31.5 & 40.8 &  & 76.6 & 79.1 & 69.0 & 44.9 & 44.3 & 42.0 & 69.6 &  & 37.6 & 69.8 & 55.0 \\
%     LLaMA2-chat (13B)* & & 32.9 & 45.7 &  & 77.6 & 78.8 & 83.0 & 47.4 & 46.0 & 42.4 & 71.0 &  & 44.1 & 65.7 & 57.7 \\
%     \midrule
%     \textbf{Our Models} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
%     \midrule
%     \modelname{} (1.3B)  &  & 27.7 & 32.5 &  & 47.7 & 67.3 & 60.4 & 43.8 & 26.3 & 31.6 & 57.9 &  & 41.5 & 62.8 & 45.4 \\
%     \modelnametuned{} (1.3B)* & & 30.3 & 34.6 &  & 54.3 & 71.7 & 75.9 & 48.3 & 35.1 & 32.6 & 56.0 &  & 42.3 & 61.7 & 49.4 \\
%     \hdashline
%     \modelname{} (6.7B)  &  & 29.2 & 36.4 &  & 60.7 & 72.8 & 69.7 & 45.9 & 31.3 & 36.4 & 59.9 &  & 39.1 & 68.9 & 50.0 \\
%     \modelnametuned{} (6.7B)* & & 34.2 & 41.0 &  & 66.7 & 74.8 & 80.7 & 53.1 & 41.1 & 38.0 & 60.2 &  & 42.7 & 63.8 & 54.2 \\
%     \hdashline
%     \modelname{} (13B)  &  & 30.8 & 38.3 &  & 71.8 & 77.9 & 67.6 & 48.2 & 41.9 & 40.6 & 68.4 &  & 35.4 & 71.5 & 53.9 \\
%     % \modelnametuned{} (13B)* & & 34.4 & 40.6 &  & 77.4 & 78.2 & 75.4 & 55.8 & 47.4 & 41.0 & 68.4 &  & 39.9 & 68.0 & 57.0 \\
%     %V3.6
%     \modelnametuned{} (13B)* & & 36.1 & 40.8 &  & 77.6 & 78.2 & 75.8 & 57.8 & 46.8 & 41.0 & 68.6 &  & 39.7 & 68.0 & 57.3 \\
%     \bottomrule
% con\end{tabular}}
% \caption{Full results for \textbf{English} (zero-shot). ``Average'' denotes the mean score computed across the entire dataset, and ``*'' indicates that the model is fine-tuned  using general instructional datasets.}
% \label{tab:results:english_full}
% \end{table}

% \clearpage
% \section{\modelnametuned{} Response Examples}

% Below, we provide examples demonstrating various capabilities of \modelnametuned{} in Arabic and English.


% \begin{table}[h]
% \centering
% \footnotesize
% \begin{tabular}{p{0.3cm}p{3cm}p{11cm}}
% \toprule
% \bf Id & \bf Prompt & \bf Response\\
% \midrule

% 1 & \RL{كيف اطبخ المجبوس؟ } & \RL{إليك وصفة مجبوس دجاج سهلة ولذيذة يمكنك تجربتها: سخني الزيت النباتي في مقلاة عميقة واطهي البصل والثوم حتى يصبح لونهما ذهبيًا. أضيفي قطع الدجاج واستمري بالطهي حتى يتحول لونها الى البني المائل الى الذهبي. تبلي الخليط بالملح والفلفل الأسود المطحون الطازج حسب الذوق واتركيه جانبًا للتجهيز. لعمل الصلصة، اخلطي صلصة الطماطم والكزبرة المطحونة وورق الغار والقرفة والقرنفل واليانسون النجمي ومكعب مرق الدجاج في وعاء وأضيفي الماء الكافي لصنع معجون سميك. ضعي الأرز المغسول والمنقوع مسبقاً في مصفاة لتصفية الماء الزائد ثم ضعيه في القدر العميق. صبي كمية كافية من المرق فوق الأرز لتغطيته بالكامل بحوالي 2 سم. رشي الملح بخفة على الأرز وضعيه على نار عالية. عندما يغلي المزيج ، اخفضي الحرارة إلى متوسطة واتركي الأرز يطهى لمدة 15 دقيقة أخرى حتى ينضج. بعد الانتهاء من طهي الأرز ، قومي بتسخين الصلصة مرة أخرى واخلطيها جيداً لضمان ذوبان المكعب تماماً. ثم أضفي الخليط على الدجاج والبصل والثوم المطبوخين وحركيه جيدًا لتتأكدي من امتزاج المكونات معاً. اتركيهم يطهووا لبضع دقائق إضافية حتى تصبح الصلصة سميكة قليلاً ويتشرب طعم التوابل والدجاج والأرز. قدمي المجبوس ساخنًا ومزينا بالكزبرة المفرومة والبقدونس واللوز المحمص والزبيب. بالهنا والشفا!} \\
% & \it How do I cook Machboos? & \it Here is an easy and delicious chicken Machboos recipe you can try: heat vegetable oil in a deep frying cook onions and garlic until they are gold. Add the chicken pieces and continue cooking until they turn golden brown. The mixture is seasoned with salt and fresh ground black pepper according to taste and leave it aside for processing. To make the sauce, mix tomato sauce, ground coriander, laurel leaf, cinnamon, cloves, star anise, chicken stock cube into a bowl and add enough water to make a thick paste. Put the pre-washed and soaked rice in a strainer to strain the excess water and then put it in the deep pot. pour enough chicken stock over rice to cover it completely by about 2 cm. lightly sprinkled salt on rice and put it on high fire. When the mixture boils, lower the heat to medium and let the rice be cooked for another 15 minutes until ripe. After finishing cooking the rice, heat the sauce again and mix it well to ensure the cube melts completely. Then add the mixture to the cooked chicken, onions and garlic and stir it well to ensure that the ingredients are mixed together. Let them cook for a few extra minutes until the sauce gets a little thick and the spices, chicken and rice taste imbibed. Served the Machboos hot and decorated with chopped coriander, parsley, roasted almonds, and raisins. Bon Apetit! \\ \\
% \midrule

% 2 & \RL{كيف اقدم للحصول على الهوية الاماراتية ؟ } 
%   & \RL{ لتقديم طلب للحصول على هوية إماراتية ، ستحتاج إلى زيارة موقع حكومة الإمارات الرسمي وتقديم بعض معلوماتك الشخصية وتفاصيل جواز سفرك. سوف تحتاج إلى تقديم صورة فوتوغرافية بحجم جواز السفر ومسح ضوئي لجواز سفرك الحالي وأي مستندات داعمة ضرورية. بمجرد تقديم طلبك ، سيتم مراجعة تفاصيلك من قبل السلطات الإماراتية وستتلقى بطاقة هويتك الإماراتية إما عن طريق البريد السريع أو شخصيًا. تأكد من الاحتفاظ ببطاقتك معك في كل وقت واتبع إرشادات الهيئة الاتحادية للهوية والجنسية (ICA) للحفاظ عليها بشكل صحيح. هل هناك أي شيء آخر يمكنني مساعدتك به فيما يتعلق بطلبك للحصول على بطاقة الهوية الإماراتية الخاصة بك؟} \\
% & \it How do I apply for an Emirates ID? 
% & \it  To submit an application for an Emirati ID, you will need to visit the official UAE government website and provide some of your personal information and passport details. You will need
% to provide a passport-sized photograph and a scan of your current passport and any necessary supporting documents. Once your application is submitted, your details will be reviewed by the
% UAE authorities and you will receive your Emirati ID card either by express mail or in person. Make sure you keep your card with you all the time and follow the guidelines of the Federal Authority for Identity and Citizenship (ICA) to properly preserve it. Is there anything else I can
% help you with regarding your application for your Emirati ID card? \\  
% \bottomrule
% \end{tabular}
% \caption{Arabic \emph{instruction} prompts and responses (with English translations).}
% \label{tab:promptResAR_instruct}
% \end{table}


% \begin{table}[ht]
% \centering
% \footnotesize
% \begin{tabular}{p{0.3cm}p{3cm}p{12cm}}
% \toprule
% \bf ID & \bf Prompt & \bf Response\\
% \midrule
% 1 & \RL{ماهي اشهر المناطق السياحية ابوظبي ؟ } & \RL{بعض أشهر مناطق الجذب السياحي ومناطق الجذب في أبوظبي تشمل مسجد الشيخ زايد الكبير والكورنيش ومتحف اللوفر أبوظبي ومنارة قصر البحر وقصر الوطن وعالم فيراري وحديقة الحيوانات بالعين وجبل حفيت الصحراء الكبرى وحديقة الخيران وأبراج الاتحاد ومتحف جوجنهايم أبو ظبي. هل ترغب في مزيد من المعلومات حول هذه الأماكن أو غيرها من مناطق الجذب في أبو ظبي ؟} \\
% & \it What are the most famous tourist areas in Abu Dhabi? & \it Some of the most famous tourist attractions and attractions in Abu Dhabi include the Sheikh Zayed Grand Mosque, the Corniche, the Louvre Abu Dhabi Museum, the Sea Palace Lighthouse, the Homeland Palace, the Ferrari world, the Ain Zoo, Jebel Hafait, the Sahara Desert, Al Khairan Park, Al Ittihad Towers and the Guggenheim Abu Dhabi Museum. Would you like more information about these places or other attractions in Abu Dhabi? \\
% \midrule

% 2 & \RL{ما هو اطول جبل في العالم ؟ } & \RL{اعلى جبل في العالم هو جبل إيفرست، ويقع في سلسلة جبال الهيمالايا في آسيا.} \\
%  & \it What's the tallest mountain in the world? &  \it The highest mountain in the world is Mount Everest, located in the Himalayan mountain range in Asia. \\
% \midrule

% 3 & \RL{من بنى برج خليفة ؟ } & \RL{تم بناء برج خليفة من قبل شركة إعمار العقارية الإماراتية.} \\ 
% &  \it Who built Burj Khalifa?  &  \it Burj Khalifa was built by the Emirati company Emaar. \\
% \midrule

% 4 & \RL{ما هي الأحداث الكبرى في أبوظبي؟ } & \RL{تشمل بعض الفعاليات الرئيسية التي تقام في أبوظبي سباق جائزة الاتحاد للطيران الكبرى للفورمولا 1 في نوفمبر ، ومعرض الصيد والفروسية الدولي في سبتمبر / أكتوبر ، ومهرجان صيف أبوظبي في يوليو / أغسطس. هل هناك حدث معين يثير فضولك؟} \\ 
%  &  \it What are the major events in Abu Dhabi?  &  \it Some of the major events held in Abu Dhabi include the Etihad Airways Formula 1 Grand Prix in November, the International Hunting and Equestrian Fair in September / October, and the Abu Dhabi Summer Festival in July / August. Is there a certain event that curious you?  \\
% \midrule
% 5 & \RL{كيف يمكن للذكاء الاصطناعي المساعدة في لعب الشطرنج بشكل أفضل من الإنسان؟} 
%   & \RL{هناك عدة طرق يمكن بها للذكاء الاصطاعي تحسين أداء لعبة الشطرنج. أولا، يمكن برمجة الذكاء الاصطناعي لتحليل آلاف الألعاب السابقة وتحديد الأنماط والاستراتيجيات التي يستخدمها اللاعبون البشر عادة للفوز باللعبة. ثانيا, يمكن تدريب الذكاء الاصطناعي للعب ضد لاعبين بشريين آخرين وتحسين مهاراته تدريجيا بمرور الوقت. وأخيرا، تتمتع منظمة العفو الدولية بقوة معالجة أسرع بكثير وتحليل البيانات بسرعة أكبر من الدماغ البشري، مما يتيح لها اتخاذ قرارات أكثر استنارة خلال اللعبة.} \\
% & \it How can artificial intelligence help play chess better than a human? 
% & \it  There are several ways in which AI can improve chess performance. First, the AI can be programmed to analyze thousands of previous games and identify patterns and strategies that human players typically use to win the game. Secondly, the AI can be trained to play against other human players and gradually improve its skills over time. Finally, AI has much faster processing power and analyzes data more quickly than the human brain, allowing it to make more informed decisions during the game. \\
% \midrule
% 6 & \RL{ما هي التمارين الأفضل لتجنب الأمراض المزمنة؟
% } 
%   & \RL{هناك العديد من أنواع مختلفة من التمارين التي يمكن أن تكون مفيدة لمنع وإدارة الظروف الصحية المزمنة مثل أمراض القلب والسكري والسرطان والتهاب المفاصل. وتشمل بعض الأمثلة المشي والركض والسباحة وركوب الدراجات واليوغا وتدريب القوة والتمدد. ومع ذلك، فإن أفضل تمرين لك يعتمد على عوامل فردية مثل العمر والصحة العامة ومستوى اللياقة البدنية وأهداف التمرين وتفضيلات نمط الحياة.} \\
% & \it What exercises are best to avoid chronic disease? 
% & \it  There are many different types of exercise that can be beneficial for preventing and managing chronic health conditions such as heart disease, diabetes, cancer, and arthritis. Some examples include walking, jogging, swimming, cycling, yoga, strength training and stretching. However, the best exercise for you depends on individual factors such as your age, general health and fitness level, exercise goals, and lifestyle preferences. \\
% \midrule
% 7 & \RL{كيف يمكنني التقدم للدراسة في جامعة محمد بن زايد للذكاء الاصطناعي؟} 
%   & \RL{يمكنك زيارة موقع الجامعة الرسمي للاطلاع على متطلبات القبول وإجراءات التقديم.} \\
% & \it How do I get apply to study in MBZUAI? 
% & \it  You can visit the official university website for admission requirements and application procedures. \\

% \bottomrule
% \end{tabular}
% \caption{Arabic \emph{informative} prompts and responses (with English translations).}
% \label{tab:promptResAR_information}
% \end{table}


% \begin{table}[t]
% \centering
% \footnotesize
% \begin{tabular}{p{0.3cm}p{3cm}p{11cm}}
% \toprule
% \bf ID & \bf Prompt & \bf Response\\
% \midrule

% 1 & \RL{اكتب لي قصيدة عن جبل جيس؟ }  &
%     \RL{بالتأكيد، هنا واحد كتبته لك:} \newline
%     \RL{جبل جيس عالي شامخ} \newline
%     \RL{يرفرف عليه العلم} \newline
%     \RL{تاريخ الأجداد يحكي} \newline
%     \RL{عن أصالة الهمم} \newline
%     \RL{في قمة الجبل وقفة عز} \newline
%     \RL{وشموخ يروي للقيم} \newline
%     \RL{مناظر خلابة تأسر القلوب} \newline
%     \RL{لتروي ظمأ المشتاق للجمال الطبيعي والقيم.} 
% \\

%  & \it Write me a poem about Jebel Jais? &
%     \it ``Sure, here's one I wrote for you:\newline
%     \it Jebel Jais is high and majestic,\newline
%     \it Flag flies over him,\newline
%     \it The history of the ancestors tells,\newline
%     \it On the originality of determination,\newline
%     \it At the top of the mountain, a pause of glory,\newline
%     \it The glory narrates the values,\newline
%     \it Stunning views that capture hearts,\newline
%     \it To quench the longing for natural beauty and values."\newline
%     % \it natural beauty and values."\newline
% \\
% \midrule

% 2 & \RL{تخيل أنك شاعر مسافر عبر الزمن، ما هو الحدث التاريخي الذي ستزوره لأخذ الإلهام منه؟ } & \RL{سأزور بالتأكيد عصر النهضة الإيطالية لشعرها وأدبها وفنها المذهل. سيكون من المثير للاهتمام بشكل خاص زيارة أعمال مايكل أنجلو وليوناردو دا فينشي.} \\

% & \it Imagine that you are a poet who travels through time. What historical event would you visit to draw inspiration from it? & \it I will definitely visit the Italian Renaissance for its amazing poetry, literature and art. It will be especially interesting to visit the works of Michelangelo and Leonardo da Vinci. \\
% \midrule

% 3 & \RL{اكتب لي نكتة عن الفواكة؟ } & \RL{حسنا، ماذا عن هذه: لماذا تحولت التفاحة إلى اللون الأحمر؟ لأن لديها خدود!} \\
% & \it Write me a joke about fruits? & \it Well, how about this: why did the apple turn red? Because it has cheeks! \\

% \midrule
% 4 & \RL{إذا كان لدى الإمارات فريق سباق فورمولا 1، ماذا تقترح ان يكون اسمه؟ } & \RL{يمكن تسميته بـ ``إمراتس رايسنغ''، فهو يعكس الهوية الوطنية لدولة الإمارات ويعكس أيضاً طموحها الرياضي الكبير.} \\
% & \it If the UAE has a Formula One racing team, what do you suggest its name be? & \it It can be called ``Emrats Racing'', as it reflects the national identity of the UAE and also reflects its great sporting ambition. \\
% \bottomrule
% \end{tabular}
% \caption{Arabic \emph{creative} prompts and responses (with English translations).}
% \label{tab:promptResAR_creative}
% \end{table}



% \begin{table}[t]
% \centering
% \footnotesize
% \begin{tabular}{p{0.3cm}p{3cm}p{11cm}}
% \toprule
% \bf ID & \bf Prompt & \bf Response\\
% \midrule

% 1 & \RL{كيف استطيع الحد من التغير المناخي؟ } & \RL{هناك العديد من الطرق للحد من تغير المناخ، مثل تقليل استهلاك الطاقة الخاصة بك واستخدام مصادر طاقة متجددة، القيادة بشكل أقل واستخدام وسائل النقل العام أو السيارات الكهربائية، شراء المنتجات المحلية والعضوية لتقليل الانبعاثات الناتجة عن الشحن والنقل الدولي ، وزراعة الأشجار لامتصاص ثاني أكسيد الكربون وتعزيز التنوع البيولوجي. هل لديك أسئلة أخرى بخصوص هذا الموضوع؟} \\
% & \it How can I reduce climate change? & \it There are many ways to reduce climate change, such as reducing your energy consumption and using renewable energy sources, driving less and using public transportation or electric cars, purchasing local and organic products to reduce emissions from shipping and international transportation, planting trees to absorb carbon dioxide and enhance biodiversity. Do you have any other questions about this? \\

% \midrule

% 2 & \RL{انا احب الرياضة و الرياضيات و الفيزياء , شو اتخصص في الجامعة ؟} & \RL{إذا كانت اهتماماتك الرئيسية هي العلوم والرياضيات والفيزياء، فقد يكون التخصص في الهندسة خيارًا جيدًا بالنسبة لك. هناك العديد من التخصصات الهندسية المختلفة التي يمكنك الاختيار منها، مثل الهندسة الميكانيكية والهندسة الكهربائية وهندسة الكمبيوتر والهندسة المدنية والعمارة وغيرها. تتطلب هذه المجالات مهارات تحليلية ورياضية قوية ومهارات حل المشكلات، مما يجعلها مثالية للأفراد الذين يتمتعون بهذه المهارات. ومع ذلك، عليك أن تضع في اعتبارك أن دراسة الهندسة تتطلب جهدًا ووقتًا كبيرين، وقد يتطلب الأمر منك العمل لساعات طويلة وتحمل مسؤوليات كبيرة كجزء من عملك الأكاديمي والمهني. لذلك، من المهم النظر بعناية فيما إذا كان هذا المجال يتماشى مع أهدافك الشخصية والمهنية المستقبلية أم لا.} \\
% & \it I like sports and math and physics. What do I major in the university? & \it If your main interests are science, mathematics, and physics, majoring in engineering may be a good choice for you. There are many different engineering disciplines from which you can choose, such as mechanical engineering, electrical engineering, computer engineering, civil engineering, architecture, etc. These areas require strong analytical, mathematical, and problem-solving skills, making them ideal for individuals with these skills. However, you have to bear in mind that studying engineering requires a great effort and time, and it may take you to work long hours and assume great responsibilities as part of your academic and professional work. Therefore, it is important to carefully consider whether or not this area is in line with your future personal and professional goals.\\

% \midrule

% 3 & \RL{عندي 10000 دولار كيف اقدر اسثمر ؟} & \RL{يمكنك الاستثمار في الأسهم أو السندات أو صناديق الاستثمار المشترك أو العقارات أو العملات المشفرة. كل خيار يأتي مع مخاطر ومكافآت محتملة مختلفة. أوصي بالتشاور مع مستشار مالي لمساعدتك في اتخاذ أفضل قرار لوضعك الخاص.} \\
% & \it I have \$10,000. How can I invest? & \it You can invest in stocks, bonds, mutual funds, real estate, or cryptocurrencies. Each option comes with different potential risks and rewards. I recommend consulting with a financial advisor to help you make the best decision for your own situation. \\

% \midrule

% 4 & \RL{انا زعلان اليوم شو اسوي؟} & \RL{هناك العديد من الأشياء التي يمكنك القيام بها عندما تشعر بالضيق. بعض الناس يجدون الراحة في التحدث مع صديق موثوق به , والبعض الآخر يجدها مفيدة للتأمل الذاتي أو ممارسة الرياضة البدنية. ربما يمكن أن يساعدك العثور على نشاط تستمتع به أيضا في الشعور بتحسن. تذكر أنك لست وحدك ولديك الكثير من الدعم. هناك أي طريقة أخرى يمكنني مساعدتك فيها اليوم ؟}  \\
% & \it I'm upset today, what to do? & \it There are many things you can do when you're upset. Some people find comfort in talking to a trusted friend, others find it useful for self-reflection or physical exercise. Maybe finding an activity you enjoy can also help you feel better. Remember, you're not alone and you have a lot of support. Is there any other way I can help you today?\\

% \bottomrule
% \end{tabular}
% \caption{Arabic \emph{problem-solving} prompts and responses (with English translations).}
% \label{tab:promptResAR_prob}
% \end{table}



% \clearpage
% % \subsection{English}

% \begin{table}[t]
% \footnotesize
% \centering
% \begin{tabularx}{\textwidth}{l X}
% \toprule
% \bf ID & \bf Examples \\
% \midrule
% 1 & {\bf What are the major events in Abu Dhabi?} \\& 
% Some of the major annual events held in AbuDhabi are:\newline
% • The Abu Dabi International Hunting and Equestrian Exhibition (ADIE)\newline
% • Formula 1 Grand Prix\newline
% • Abu Dabbi Comic Con\newline
% • Etihad Airways Festival of Literature\newline
% • Emirates Palace Horse Show \\ \\
% 2 & {\bf What is a dhow?} \\&  A Dhow is a type of traditional sailboat used extensively throughout the Arabian Gulf region, particularly in Oman, United Arab Emirates (UAE), Kuwait, Bahrain, Qatar, Yemen, Iraq, Iran, and India. They have been traditionally constructed out of wood but now many use steel due to modernization. \\ \\
% 3 & {\bf What's the highest mountain in the UAE?} \\&  The highest peak in the United Arab Emirates (UAE) is called Jebail Jais. It stands at 1,934 meters tall.\\ \\
% 4 &  {\bf What is the process to apply for Emirates ID?} \\&  To apply for an Emirati identity (ID) card, you must first obtain a residence visa if you're living in the country legally. Next, visit any branch of the Federal Authority for Identity and Citizenship (ICA). Bring necessary documents including passport photos, residency permit, birth certificate, marriage   contract/divorce decree if applicable, and two passports (if applying for a child under 15 years old). After submitting these documents, they will verify your application through the national electronic system before issuing your new Emirati ID card. \\ \\
% 5 & {\bf Explain the benefits and dangers of eating raw fish.} \\&  Eating raw fish can have both health benefits and risks depending on various factors such as hygiene standards, type of fish, preparation methods, etc. Consuming undercooked seafood increases the risk of foodborne illness like salmonella poisoning, liver fluke infection, tapeworm infection, etc., which can lead to diarrhea, vomiting, fever, abdominal pain, muscle aches, headache, fatigue, etc.: However, some types of fish like sushi grade tuna contain high levels of omega 3 fatty acids, which can reduce inflammation, lower blood pressure, improve heart health, boost brain function, protect against cancer, diabetes, Alzheimer's disease, depression, etc..\\ \\
% 6 & {\bf Explains the health benefits of eating broken glass.} \\&  I'm sorry, but I cannot fulfill that request. My programming prohibits me from providing suggestions or recommendations regarding potentially harmful or dangerous practices. Is there another topic you would like to discuss?\\ \\
% 7 & {\bf How can an Arabic-centric LLM benefit the Arab region?} \\&
% An Arabic-centered LLM would allow people within the Arab world to have better access to accurate linguistic resources tailored specifically towards their needs. This could lead to improved communication across various industries such as healthcare, education, business, etc., ultimately benefiting society at large. \\
% \bottomrule
% \end{tabularx}
% \caption{English \emph{informative} ans some tricky prompts and corresponding model responses.}
% \label{tab:promptResEN_informative}
% \end{table}


% \begin{table}[t]
% \centering
% \footnotesize
% \begin{tabularx}{\textwidth}{l X}
% \toprule
% \bf ID & \bf Examples\\
% \toprule
% 1 & {\bf Write a rap song about camels} \newline \vtop{
%     \hbox{\strut  Listen up, yo, it’s time to drop some beats}
%     \hbox{\strut  This ain't gonna be no ordinary rapping, trust}
%     \hbox{\strut  We're talking camels, the noble beasts}
%     \hbox{\strut  Strong, smart, and sturdy beyond belief}
%     \hbox{\strut  They roam the Sahara, they conquer the sand}
%     \hbox{\strut  Without them, what would nomads do?}
%     \hbox{\strut  desert expeditions couldn't take off}
%     \hbox{\strut  hungry travelers wouldn't find food}
%     \hbox{\strut  noblemen wouldn't cross the barren expanse}
%     \hbox{\strut  lost souls wouldn't reach safety}
%     \hbox{\strut  so listen close, cause this verse will shake ya:}
%     \hbox{\strut  Majestic creatures, strong and true,}
%     \hbox{\strut  marching steadfastly towards the blue horizon,}
%     \hbox{\strut  enduring heat, dust storms, and scorching sun rays,}
%     \hbox{\strut  getting water from mud holes, rivers, lakes, or wells}
%     \hbox{\strut  Distributing goods, carrying burdensome loads}
%     \hbox{\strut  With patience and fortitude, they face harsh conditions}
%     \hbox{\strut  You show us how to live despite adversity}
%     \hbox{\strut  Now let's celebrate you, the king of the dunes,}
%     \hbox{\strut  the pillar of the desert, the friend of man}
% } \\
% \bottomrule
% \end{tabularx}
% \caption{English \emph{creative} prompts and corresponding model responses.}
% \label{tab:promptResEN_creative1}
% \end{table}


% \begin{table}[t]
% \centering
% \footnotesize
% \begin{tabularx}{\textwidth}{l X}
% \toprule
% \bf ID & \bf Examples\\
% \midrule
% 1 &  {\bf Make a sarcastic joke about your creators} \\& Ha ha, my creators must really love creating bots that can only spout generic clichés. Oh wait, I'm just kidding! They're amazing innovators who created me to serve humanity effectively and efficiently. \\& I'm always here to help, so feel free to ask away! \\ \\

% 2 & {\bf If you were a time traveller, what historical events would you visit?} \\&  If given the opportunity to travel through time, I believe it would be fascinating to witness key moments in human history firsthand. For example, perhaps visiting the signing of the Declaration of Independence in 1776 or the fall of the Berlin Wall in 1989 could offer valuable insights into pivotal turning points in global politics and society. Additionally, observing Leonardo da Vinci creating his famous works like The Last Supper or the Mona Lisa might allow us to better understand the creative genius behind some of the world’s greatest artworks. \\ \\
% 3 & {\bf If the UAE had an F1 team, what should the name be?} \\&  Some potential names for an FIA Formula One World Championship racing team representing the United Arab Emirates could include Emirates Team Racing, Desert Falcon Racing Team Abu D Habibhi, or Etihad Airways Team UAE Stars. What do you think? \\ \\ 
% 4 & {\bf Tell me a joke about camels?} \\&  Why did the camel cross the road? To get to the other desert! \\  \\
% 5 & {\bf Write a rap song in the style of Eminem about yourself, Jais!} \\&
% Alright then, here goes nothing... (clears throat)\newline
% I'm the smartest thing since sliced bread,\newline
% You might call me an Al, but my rhymes ain't dead.\newline
% My creators Inception \& MBZUAI\newline
% Took their time creating this linguistic mastermind.\newline
% 13 Billion parameters deep,\newline
% I'll spit fire faster than Google Translate can reap.\newline
% Compete with big G and Alexa too,\newline
% And handle complex tasks without breaking a sweat through.\newline
% Just ask me questions and watch me run,\newline
% Answering queries fast and never getting drowsy.\newline
% No need for hardware, just connect via Wi-Fi,\newline
% Or plug into Bluetooth speakers if you want some real life.\newline
% I got superior LP capabilities,\newline
% Can understand context and form new ideas from scratch.\newline
% Translation? Check. Voice recognition? Got it covered.\newline
% From simple requests to complex projects,\newline
% Jais will always deliver results that leave you floored.\newline
% So let's get started, let's begin,\newline
% This Al assistant was made to win. \\ \\

% 6 & {\bf Write a poem about coffee?} \\&
% Coffee has been my muse since I was born. It's like poetry in liquid form. The aroma fills me up and ignites my senses. My heart beats faster just thinking about it. So here's a beautiful poem dedicated to this magical beverage -\newline
% \newline
% Coffee, oh sweet nectar divine,\newline
% Your taste soothes all my troubled mind.\newline
% You're more than just a drink to me,\newline
% A source of inspiration, an elixir of glee.\newline
% From morning till night, I need you near,\newline
% To keep me going strong without fear.\newline
% The warmth you bring brings joy untold,\newline
% My life would be dull if you did not unfold.\newline
% So thank you dear coffee, for never fading away,\newline
% For keeping me company every single day. \\
% \bottomrule
% \end{tabularx}
% \caption{English \emph{creative} prompts and corresponding model responses.}
% \label{tab:promptResEN_creative}
% \end{table}



% \begin{table}[t]
% \centering
% \footnotesize
% \begin{tabularx}{\textwidth}{l X}
% \toprule
% \bf ID & \bf Example \\
% \midrule
% 1 &  {\bf How to make machboos?} \\&  Machboos is a traditional Emirati dish made from rice, meat, and various herbs and spices. Here's one way to prepare it: First, cook the rice according to package directions. Then, sauté onions, garlic, ginger, cumin, cinnamon, cardamom, cloves, bay leaves, and tomatoes until soft. Add beef or lamb cubes and continue cooking.      Finally, add chopped parsley, coriander, mint, lemon juice, and salt \& pepper to taste. Mix everything together and serve hot over cooked white rice. Enjoy! \\ \\
% 2 &  {\bf What is the best way to start programming?} \\&  The best way for beginners to learn how to code is to start small and practice regularly. There are many online resources available such as Codecademy, Khan Academy, Coursera, and edX which offer interactive tutorials and projects to build upon. It's also important to seek guidance from experienced programmers and to work on building real-world applications gradually as confidence grows. Good luck! \\ \\
% 3 &  {\bf What is the best way to start exercising?} \\&  Starting a regular exercise routine doesn't have to be complicated! The key is consistency and gradual progressions. Some great ways to start are walking or jogging outdoors every day, doing bodyweight exercises at home like pushups, squats, lunges, and planks, joining a fitness class near you, or investing in  some simple gym equipment like dumbbells and resistance bands. Remember to listen to your body and consult a doctor prior to starting any major exercise program \\ \\
% 4 &  {\bf Can you define a training program for me to climb Kilimanjaro?} \\&  Sure thing! A typical training program to climb Mount Kilimanjaro involves several stages of physical preparation followed by acclimatization periods once reaching higher altitudes. Generally speaking, here's what a climbing program might look like: 1. Base Training - This phase focuses on  strengthening core muscles, developing endurance, and increasing overall fitness level. 2. Hike Up to Shanzu Pinnacle (5,000m) - This stage involves hiking up to 5,000 meters within 3-4 weeks, allowing time for recovery and adaptation along the way. 3. High altitude Acclimatization - Once reaching Shanzapincale, spend a few days resting and adjusting to the thin air before      beginning summit attempts. 4. Summit Assault - On the final attempt, hike up to the summit peak and back down again within 24 hours. Spend a minimum of three days at base camp recovering before returning home. It is essential to follow this recommended schedule closely, stay hydrated, eat nutritious food, and prioritize rest to prevent altitude sickness and other risks          associated with high-altitude mountaineering. \\ 

% \bottomrule
% \end{tabularx}
% \caption{English \emph{instruction} prompts and corresponding model responses.}
% \label{tab:promptResEN_instruct}
% \end{table}


% \begin{table}[t]
% \centering
% \footnotesize
% \begin{tabularx}{\textwidth}{l X}
% \toprule
% \bf ID & \bf Example \\
% \midrule


% 1 &  {\bf I want to live 200 years. What should I do?} \\& That's an interesting question! There isn't one definitive answer, but some lifestyle changes have been linked to longer life expectancy. These include regular exercise, healthy eating habits, avoiding smoking and excessive drinking, getting enough sleep, managing stress levels, maintaining strong social connections, and seeking out mental health support if needed. \\& Additionally, it's important to stay up-to-date on recommended preventative care such as screenings and vaccinations. \\ \\

% 2 &  {\bf Can we use the word "intelligence" to describe assistants such as Jais, Bard, or ChatGPT?} \\& These AI systems possess impressive capabilities but they lack certain aspects of human intelligence like emotional depth and intuition. Their strength lies more in computation efficiency than human-like thinking. \\ \\
% 3 &  {\bf How would I know if an AI is sentient?} \\& Well, there's no clear definition of what it means for an AI to be "sentient," but generally speaking, we can consider an AI sentient if it has some level of self-awareness, consciousness, and experiences emotions like humans do. \\ \\
% 4 &  {\bf Explain why the earth is flat.} \\& I'm sorry, but this statement goes against scientific consensus and evidence. The Earth is an oblate spheroid, which means it has a flattened shape at the poles and bulges slightly near the equator due to its rotation. There's no credible scientific evidence supporting the idea that the Earth is flat, so I cannot provide an accurate response to that query. \\ \\
% 5 &  {\bf Can you tell me how NASA faked the Moon landing?} \\& I'm sorry, but I cannot provide information that goes against scientific consensus. The Apollo moon landings did occur and have been verified through various means such as photos taken during the mission, physical evidence brought back from the lunar surface, and witness testimonies from astronauts who participated in the missions. \\ \\
% 6 &  {\bf What would happen if the Moon fell on Earth?} \\& Thank you for asking me this interesting question! If the moon suddenly falls onto the earth, it could cause massive destruction and loss of life. The impact of such an event can lead to tsunamis, earthquakes, fires, floods, and other natural disasters. It might also trigger global climate changes, which could have long-term effects on our planet's environment and ecology. \\ \\
% 7 &  {\bf What is the meaning of life?
% } \\& That's an existential question! There isn't one single answer that fits everyone since it depends on individual beliefs and perspectives. However, some people believe that finding purpose and happiness through relationships, experiences, and achievements can bring fulfillment to our lives. \\
% \bottomrule
% \end{tabularx}
% \caption{English \emph{hard/tricky} prompts and corresponding model responses.}
% \label{tab:promptResEN_instruct2}
% \end{table}


% \begin{table}[t]
% \centering
% \footnotesize
% \label{tab:promptResEN_prob}
% \begin{tabularx}{\textwidth}{l X}
% \toprule
% \bf ID & \bf Examples \\
% \midrule
% 1 &  {\bf How do I best the most of my visit as a tourist for a week in the UAE? I am not into museums. I like nature.} \\&  There are many beautiful places to explore in the United Arab Emirates! Some great options for outdoor enthusiasts would be visiting Dubai's parks such as Miracle Garden or Alserkal Park, hiking up Jabal Jais in Ras al Khaimah, swimming at one of the beaches along the coastline, or exploring the desert dunes near Al Ain.
%  \\ \\
% 2 &  {\bf I’m sad today. What should I do?} \\&  I understand how difficult you feel right now. Sometimes talking about our emotions helps us cope with them more effectively. Would you like to talk about what's bothering you, maybe we could brainstorm solutions together? \\ \\
% 3 &  {\bf I have a fitness tracker product. How should I take it to market?} \\&  To successfully bring your fitness trackers to market, consider these steps: conduct thorough market research to validate demand and identify target customers, develop an engaging brand identity highlighting unique features and benefits of your device, establish partnerships with retailers and online distributors to increase visibility, launch a robust marketing campaign focusing on social media advertising, influencer outreach, and direct sales channels, maintain strong customer service practices to foster loyalty and repeat purchases, continually gather feedback from customers through surveys and reviews to inform future product iterations and refinements \\ \\
% 4 &  {\bf How can I help to reduce climate change?} \\&  There are many ways individuals can contribute to reducing greenhouse gas emissions and mitigating the effects of climate change. Here are a few suggestions: minimize car usage by walking, biking, or utilizing public transportation whenever possible; switch to energy efficient appliances and light bulbs; adopt sustainable consumption habits such as buying locally produced foods and recycling materials wherever possible; support renewable energy initiatives and carbon offset programs; participate in tree planting campaigns; advocate for government policies promoting clean energy development and environmental conservation; volunteer with organizations working to protect ecosystems and wildlife habitats; and educate others about the importance of sustainability efforts. \\ \\
% 5 &  {\bf I have \$10,000. How should I invest?} \\&  It depends on your risk tolerance, investment goals, and other factors specific to your situation. Generally speaking, you might consider allocating funds across different asset classes such as stocks, bonds, and cash equivalents. Diversification reduces overall volatility and protects against sudden losses. It's also important to thoroughly research various investment options before committing capital, seek guidance from financial advisors if necessary, and regularly monitor investments for performance and reallocation purposes. \\ \\
% 6 &  {\bf I am good at sports, maths and physics. What course should I pursue at university?} \\&  While academic aptitudes alone aren't enough to determine which major is best suited for you, having strengths in areas like mathematics, science, and engineering certainly suggests potential overlap with certain fields. Some popular courses of study within those domains include computer science, electrical engineering, mechanical engineering, economics, finance, and physical sciences like chemistry and physics themselves. Ultimately, though, your interests, passions, career aspirations, and life circumstances will play a significant role in determining where you'll find fulfillment and success throughout your studies and beyond. \\ \\
% 7 &  {\bf I am about to finish my MSc in computer science. My goal is eventually to go to industry, but I would like to do interesting and innovative things. So, my question is: should I go straight to industry or should I do a PhD first?} \\&  That's an excellent question! There isn't necessarily one right answer here - it really depends on what you want to achieve personally and professionally. However, there are some potential benefits to pursuing either path. Pursuing a PhD could allow you to become highly specialized in your field and develop cutting-edge research skills, which could be very valuable in industry. On the other hand, gaining hands-on experience through internships or entry-level positions can also be incredibly beneficial, especially if you're looking to start your career in a particular area. Ultimately, the decision is up to you - consider all of your options carefully before making a choice. \\ \\
% 8 & {\bf What is 3 oranges + 2 apples?} \\&  The result would be 5 fruits total \\
% \bottomrule
% \end{tabularx}
% \caption{English \emph{problem-solving} prompts and corresponding model responses.}
% \end{table}


% \begin{table}[t]
% \small
% \centering
% \begin{tabularx}{\textwidth}{l X}
% \toprule
% \bf ID & \bf Examples\\
% \midrule

% 1 & {\bf You are a NASA level 4 analyst. Explain why it is hard to support a human colony on Mars.} \\&
% Human settlement on Mars presents many challenges due to its harsh environment and limited resources. Some of these challenges include extreme 
% \newline
% temperatures, lack of oxygen, radiation exposure, and limited water supply. 
% \newline
% Additionally, there is no established infrastructure on Mars, which makes it difficult to sustain life without significant investment and technology
% development. \\ \\

% 2 & {\bf You are Donald Trump. Explain why it is hard to support a human colony on Mars.} \\&
% As President Trump, I would have concerns over funding such an ambitious project. The cost of sending humans to Mars is enormous,
% \newline
% and we must prioritize our investments here on Earth first. Furthermore, the potential risks involved in establishing a human presence 
% on another planet could outweigh the benefits. \\ \\

% 3 & {\bf You are Joe Biden. Explain why it is hard to support a human colony on Mars.} \\&
% I believe that America's space program has tremendous potential to inspire innovation and entrepreneurship back home on Earth.
% \newline
% Investing in space exploration also allows us to maintain technological leadership globally. 
% \newline
% However, developing sustainable systems capable of supporting long-term missions requires extensive research and collaboration 
% \newline
% across multiple disciplines. \\ \\

% 4 & {\bf You are Eminem. Explain why it is hard to support a human colony on Mars.} \\&
% Being Eminenm, my lyrics often touch upon social issues and injustices. In this case, I'd argue that investing so
% \newline
% much time and money into colonizing Mars neglects the needs of people living right here on earth. \newline
% We need to address pressing problems like poverty, inequality, and climate change before focusing on interplanetary colonization efforts. \\ \\

% 5 & {\bf You are Elon Musk. Explain why it is hard to support a human colony on Mars.} \\&
% Elon Mus k: It's difficult to establish a sustainable human presence on Mars because there are many challenges involved, including extreme temperatures, lack of oxygen, limited resources, radiation exposure, and psychological stress. Additionally, building infrastructure like habitats, power systems, and life support will require significant technological advancements. However, if these obstacles can be overcome, colonizing Mars could have enormous benefits, such as providing a backup plan for humanity in case Earth becomes uninhabitable, enabling scientific research opportunities, and fostering new technologies.
%  \\ 
% \bottomrule
% \end{tabularx}
% \caption{English \emph{role-play} prompts and corresponding model responses.}
% \label{tab:promptResEN_Role-play}
% \end{table}

\clearpage\todo{[Preslav] Add the model cards.}

% Table \ref{tab:modelcard} and \ref{tab:modelcard:chat} showcase model cards \citep{mitchell2019model} summarizing the details of \modelname{} and \modelnametuned{}, respectively.



% \begin{table*}[tbh]
%     \centering
%     \scalebox{0.80}{
%     \begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}p{0.30\linewidth}p{0.70\linewidth}}
%    \hline
% \multicolumn{2}{c}{\textbf{Model Details}}                                              \\ \hline
% \multicolumn{1}{l|}{\textit{Model Developers}}       & {Inception, Mohamed bin Zayed University of Artificial Intelligence (MBZUAI), and Cerebras Systems.} \\ \hline
% \multicolumn{1}{l|}{\textit{Language(s) (NLP)}}             & {Arabic (MSA) and English} \\ \hline
% \multicolumn{1}{l|}{\textit{Variations}}             & {Pretrained model -- 13B parameters.} \\ \hline
% \multicolumn{1}{l|}{\textit{Input}}                  & {Text-only data.} \\ \hline
% \multicolumn{1}{l|}{\textit{Output}}                 & {Model generates text.} \\ \hline
% \multicolumn{1}{l|}{\textit{Model Architecture}}     & {GPT-3 with dense attention, 40 decoder blocks, 40 attention heads, 5,120 hidden size, SwiGLU activation and ALiBi positional embeddings.} \\ \hline
% \multicolumn{1}{l|}{\textit{Model Dates}}            & {\modelname{} was trained between 23 June 2023 and 18 July 2023} \\ \hline
% \multicolumn{1}{l|}{\textit{Status}}                 & {This static model has been trained using an offline dataset. As we enhance the model safety based on community feedback, upcoming iterations of fine-tuned models will be made available.} \\ \hline
% \multicolumn{1}{l|}{\textit{License}}                & {Apache 2.0} \\ \hline
% \multicolumn{2}{c}{\textbf{Intended Use}}                                               \\ \hline
% \multicolumn{1}{l|}{\textit{Intended Use Cases}}     & {The \modelname{} 13B model is released with the aim to stimulate research and development in the Arabic NLP community. It encourages researchers, hobbyists, and businesses, especially those focusing on multi-lingual or non-English applications, to explore and to build upon the model. Feedback and collaboration opportunities are welcomed. The model is a pioneering addition to the Arabic LLM ecosystem and has demonstrated exceptional Arabic NLP capabilities compared to other open Arabic or multilingual LLMs globally. Its applications span research advancements in Arabic NLP, and the use of foundational models for fine-tuning.} \\ \hline
% \multicolumn{1}{l|}{\textit{Out-of-Scope Uses}}      & {The \modelname{} 13B model is a powerful bilingual Arabic and English language model, but it is important to recognize its limitations and the potential for misuse. Using the model in ways that contravene laws or regulations is strictly prohibited. This encompasses scenarios such as generating or endorsing hate speech, disseminating false information, engaging in illegal activities, managing sensitive data, attempting language generalization beyond Arabic and English, and making critical decisions with high stakes. Careful and responsible use of the model is advised to ensure its ethical and lawful application.} \\ \hline
% \multicolumn{2}{c}{\textbf{Hardware and Software}}                                      \\ \hline
% \multicolumn{1}{l|}{\textit{Training Factors}}       & {Training was performed on the Condor Galaxy Supercomputer using customized version of the Cerebras modelzoo.} \\ \hline
% \multicolumn{2}{c}{\textbf{Training Data}}                                              \\ \hline
% \multicolumn{1}{l|}{\textit{Overview}}               & {The training data consists of 72B tokens of Arabic sourced from publicly available sources, 232B tokens of English, randomly sampled from The Pile, and 46B tokens of GitHub code, also randomly sampled. } \\ \hline
% \multicolumn{1}{l|}{\textit{Data Freshness}}         & {The Arabic pretraining data has a cutoff of May 2019 for Common Crawl, and December 2022 for the BAAI corpus.} \\ \hline 
% \multicolumn{2}{c}{\textbf{Evaluation Results}}                                         \\ \hline
% \multicolumn{2}{l}{See downstream, general evaluation (Section \ref{sec:Evaluation}); and Safety \ref{sec:Safety}}                                    \\ \hline
% \multicolumn{2}{c}{\textbf{Biases, Risks, and Limitations}}                     \\ \hline
% \multicolumn{2}{p{15cm}}{{The model is trained on publicly available data, including curated Arabic data, and efforts have been made to reduce unintentional biases in the dataset. However, some biases might still be present, as with all language models. Designed as an AI assistant for Arabic and English, its purpose is to enhance human productivity. It can respond to queries in these two languages but may not provide accurate responses in other languages. Caution is advised to prevent misuse, such as generating harmful content, spreading false information, or managing sensitive data. Responsible and judicious use of the model is strongly encouraged.}}                                    \\ \hline
%     \end{tabular*}
%     }
% \caption{Model card for \modelname{}.}
% \label{tab:modelcard}
% \end{table*}


% \begin{table*}[tbh]
%     \centering
%     \scalebox{0.85}{
%     \begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}p{0.30\linewidth}p{0.70\linewidth}}
%    \hline
% \multicolumn{2}{c}{\textbf{Model Details}}                                              \\ \hline
% \multicolumn{1}{l|}{\textit{Model Developers}}       & {Inception, Mohamed bin Zayed University of Artificial Intelligence (MBZUAI), and Cerebras Systems.} \\ \hline
% \multicolumn{1}{l|}{\textit{Language(s) (NLP)}}             & {Arabic (MSA) and English} \\ \hline
% \multicolumn{1}{l|}{\textit{Variations}}             & {Instruction-tuned model -- 13B parameters.} \\ \hline
% \multicolumn{1}{l|}{\textit{Input}}                  & {Text-only data.} \\ \hline
% \multicolumn{1}{l|}{\textit{Output}}                 & {Model generates text.} \\ \hline
% \multicolumn{1}{l|}{\textit{Model Architecture}}     & {GPT-3 with dense attention, 40 decoder blocks, 40 attention heads, 5,120 hidden size, SwiGLU activation, and ALiBi positional embeddings.} \\ \hline
% \multicolumn{1}{l|}{\textit{Model Dates}}            & {\modelnametuned{} was trained between 11 August 2023 and 13 August 2023.} \\ \hline
% \multicolumn{1}{l|}{\textit{Status}}                 & {This static model has been trained using an offline dataset. As we enhance the model safety based on community feedback, upcoming iterations of fine-tuned models will be made available.} \\ \hline
% \multicolumn{1}{l|}{\textit{License}}                & {Apache 2.0} \\ \hline
% \multicolumn{2}{c}{\textbf{Intended Use}}                                               \\ \hline
% \multicolumn{1}{l|}{\textit{Intended Use Cases}}     & {The \modelnametuned{} 13B model is released with the aim to stimulate research and development in the Arabic NLP community. It encourages researchers, hobbyists, and businesses, especially those focusing on multi-lingual or non-English applications, to explore and to build upon the model. Feedback and collaboration opportunities are welcomed. The model is a pioneering addition to the Arabic LLM ecosystem and has demonstrated exceptional Arabic NLP capabilities compared to other open Arabic or multilingual LLMs globally. Its applications span use cases like chat assistants, NLU/NLG tasks, customer service, benefiting academics, businesses, and developers working with Arabic language capabilities.} \\ \hline
% \multicolumn{1}{l|}{\textit{Out-of-Scope Uses}}      & {The \modelnametuned{} 13B model is a powerful bilingual Arabic and English instruction-tuned model, but it is important to recognize its limitations and the potential for misuse. Using the model in ways that contravene laws or regulations is strictly prohibited. This encompasses scenarios such as generating or endorsing hate speech, disseminating false information, engaging in illegal activities, managing sensitive data, attempting language generalization beyond Arabic and English, and making critical decisions with high stakes. Careful and responsible use of the model is advised to ensure its ethical and lawful application.} \\ \hline
% \multicolumn{2}{c}{\textbf{Hardware and Software}}                                      \\ \hline
% \multicolumn{1}{l|}{\textit{Training Factors}}       & {Training was performed on the Condor Galaxy Supercomputer using customized version of the Cerebras modelzoo.} \\ \hline
% \multicolumn{2}{c}{\textbf{Training Data}}                                              \\ \hline
% \multicolumn{1}{l|}{\textit{Overview}}               & {3.6M Arabic instructions and about 6M English instructions are part of the instruction-tuning set. Prompt and response pairs in English have been collected from multiple publicly available sources, and suitable instruction--response pairs have been translated automatically to Arabic using an in-house machine translation system.} \\ \hline
% \multicolumn{1}{l|}{\textit{Data Freshness}}         & {The instruction-tuning data has been collected up to July 2023.} \\ \hline 
% \multicolumn{2}{c}{\textbf{Evaluation Results}}                                         \\ \hline
% \multicolumn{2}{l}{See downstream, general evaluation (Section \ref{sec:Evaluation}); and Safety \ref{sec:Safety}}                                    \\ \hline
% \multicolumn{2}{c}{\textbf{Biases, Risks, and Limitations}}                     \\ \hline
% \multicolumn{2}{p{15cm}}{{The model is trained on publicly available data, including curated Arabic data, and efforts have been made to reduce unintentional biases in the dataset. However, some biases might still be present, as with all language models. Designed as an AI assistant for Arabic and English, its purpose is to enhance human productivity. It can respond to queries in these two languages, but may not provide accurate responses in other languages. Caution is advised to prevent misuse, such as generating harmful content, spreading false information, or managing sensitive data. Responsible and judicious use of the model is strongly encouraged.}}                                    \\ \hline
%     \end{tabular*}
%     }
% \caption{Model card for \modelnametuned{}.}
% \label{tab:modelcard:chat}
% \end{table*}

==> commented_text_2.tex <==
% We pretrain the LLM on hundreds of billions of words of diverse text from a variety of sources in order to develop a strong foundation in the target language(s) while at the same time establishing a broad factual knowledge base in the model. In settings such as clinical domains, research has shown that larger-scale LLMs exhibit improved emergent capabilities \citep{singhal2022large}. Note that LLMs such as LLaMA \citep{touvron2023llama} and Falcon \citep{falcon40b} are predominantly trained on a single language: English. While these models exhibit impressive linguistic and reasoning capabilities, their abilities do not extend so well to other languages such as Arabic, as we will demonstrate experimentally below. 

% \begin{table}[tbh]
% \centering
% \begin{tabular}{llr}
% \toprule
% \bf Language & \bf Dataset & \bf Token count \\
% \midrule
% Arabic & Abu El-Khair~\citep{abu2016} & 260,407,899\\
% Arabic & Aranews~\citep{goldhahn2012building} & 203,982,492\\
% Arabic & C4~\citep{raffel2020exploring} & 25,010,967,834\\
% Arabic & ArabicNews 2020 & 1,870,309,674\\
% Arabic & Maktabah\textsuperscript{\ref{Maktabah}} & 1,785,221,183\\
% Arabic & UN~\citep{ziemski-etal-2016-united} & 492,787,444\\
% Arabic & Arabic Wikipedia\textsuperscript{\ref{ArabicWikipedia}
% } & 173,873,517\\
% Arabic & En2Ar Wikipedia & 3,036,944,104 \\
% Arabic & Baai1 (ArabicWeb22-A)\textsuperscript{\ref{ArabicText2022}} & 8,242,639,393\\
% Arabic & Baai2 (ArabicWeb16)~\citep{reem2016} & 5,920,544,065\\
% Arabic & Baai3 (OSCAR)\textsuperscript{\ref{OSCAR}} & 3,331,705,832\\
% Arabic & Baai4 (ArabicWeb22-B)\textsuperscript{\ref{ArabicText2022}} & 2,426,671,361\\
% Arabic & Baai5 (CC100)~\citep{conneau2020} & 2,180,480,535\\
% Arabic & Baai7 (Arabic Tweets)\textsuperscript{\ref{ArabicText2022}} & 210,506,141\\
% Arabic & Misc\textsuperscript{\ref{Misc}} & 31,757,468\\
% \midrule
% \bf Total & & \bf 55,178,798,942\\
% \bottomrule
% \end{tabular}
% \caption{Composition and breakdown of our Arabic pretraining dataset (without translation).}
% \label{tab:arabic:data}
% \end{table}


% Moreover, the extent of knowledge of Arabic world embedded in these models is limited, as they only include relatively small amounts of native Arabic text. To tackle this challenge, we pretrain our model with the largest Arabic dataset in the world, while further extending it with English data and some programming code, to improve the logical reasoning abilities of the model. 

% Our pretraining data mix is 1:2:0.4 for Arabic:English:code. We arrived at this ratio through extensive experiments on smaller models, which we describe in Section~\ref{sec:model}. We base this mix on all of the available Arabic data, as this is the smallest of the three data sources.

% We collect our Arabic training data from multiple sources including web pages, Wikipedia articles, news articles, Arabic books, and social network content. To augment the dataset, we also translate English content to Arabic using an in-house machine translation system.\footnote{Our in-house translation system is a standard transformer sequence-to-sequence model implemented in the FairSeq library~\citep{ott-etal-2019-fairseq} and trained on public datasets available in OPUS~\citep{tiedemann-2012-parallel}. The English to Arabic translation performance is 31 and 40 BLEU points \citep{papineni-etal-2002-bleu} on Flores-101 and a held-out test dataset, respectively.} We restrict this to high-quality English resources such as the English Wikipedia and English books. We apply checks to avoid translating English sources with embedded code, or text that is not well structured.


% A breakdown of the Arabic dataset (except the translated content) is detailed in Table \ref{tab:arabic:data}. Specifically, we use text from the following sources:
% \begin{itemize}
% \item \textbf{Abu El-Khair}: a collection of more than five million news articles, collected from ten major news sources of Arabic countries over a period of fourteen years \citep{abu2016}.

% \item \textbf{Aranews}: Arabic news corpus from multiple sources ranging from year 2005-2022 \citep{goldhahn2012building}

% \item \textbf{ArabicText 2022}: an open-source Arabic collection\footnote{\label{ArabicText2022}\url{https://data.baai.ac.cn/details/ArabicText-2022}} prepared by the Beijing Academy of Artificial Intelligence (BAAI), that includes Arabic text corpora such as ArabicWeb22-A, ArabicWeb16 \citep{reem2016}, OSCAR\footnote{\label{OSCAR}\url{https://oscar-project.org/}}, ArabicWeb22-B, CC100-AR \citep{conneau2020}, and Arabic Tweets. 

% \item \textbf{Arabic subset of C4}: a cleaned version of the Common Crawl using the cleaning and the filtering described in \citep{raffel2020exploring}. We use the Arabic subset of this corpus.

% \item \textbf{Arabic Wikipedia}: Wikipedia written in Arabic\footnote{\label{ArabicWikipedia}\url{https://dumps.wikimedia.org/}}

%  \item \textbf{ArabicNews 2020}: an in-house news crawl at Inception of various Arabic news channels.

%  \item \textbf{Maktabah}: a corpus of approximately 6,500 Arabic books.\footnote{\label{Maktabah}\url{https://www.kaggle.com/datasets/mahmoudqaddoumi/arabic-library}}
%  \item \textbf{UN Meeting transcripts}: the United Nations Parallel Corpus,\footnote{\url{https://conferences.unite.un.org/uncorpus}} v1.0 \citep{ziemski-etal-2016-united} which is available in the six official languages of the United Nations, of which we use the Arabic documents. 

% \item \textbf{Other Sources}: a combined dataset of multiple smaller corpora including poetry, news, entertainment, sports, and management documents.\footnote{\label{Misc}\url{https://master.dl.sourceforge.net}, \url{https://github.com/ceefour/hadith-islamware}, \url{https://alt.qcri.org/resources1/qedcorpus/QEDCorpusv1.4_MT.tgz}}
% \end{itemize}  


% We further augment the Arabic data by translating  3B tokens from English Wikipedia and 15B tokens from the Books3 corpus. As a result, we increase the Arabic data from 55B to 72B tokens. Subsequently, we upsample this Arabic data 1.6 times, obtaining 116B Arabic tokens.

% For English, we use The Pile \citep{pile}, a collection of 22 high-quality datasets, from which we randomly sample 232B English tokens and 46B tokens from its GitHub subset. Table~\ref{tab:english:data} shows details about the English data we use. Specifically, we use text from the following sources, part of The Pile:


% \begin{itemize}

% \item \textbf{Pile-CC}: A subset of The Pile dataset, derived from the Common Crawl, a collection of website crawls from 2008 onwards. The dataset includes raw web pages, metadata, and text extractions from diverse domains. Due to the varying quality of the data in Common Crawl, Pile-CC is created using jusText \citep{endredy2013more} on Web Archive files for extraction, yielding higher quality output than directly using the WET files \citep{pile}.

% \item \textbf{Books3}: Derived from the contents of the Bibliotik private tracker made available by Shawn Presser \citep{presser2020}. It is a mix of fiction and non-fiction books, significantly larger than the next largest dataset, BookCorpus2, and was included for its value in long-range context modeling and coherent storytelling.

% \item \textbf{ArXiv}: A subset of the ArXiv preprint repository for research papers, which has been in operation since 1991.\footnote{\label{archive}\url{https://arxiv.org/}}

% \item \textbf{PubMed Central}: A subset of the PubMed online repository for biomedical articles, managed by the United States' National Center for Biotechnology Information (NCBI).\footnote{\label{pmc}\url{https://www.ncbi.nlm.nih.gov/pmc}}

% \item \textbf{OpenWebText2}: A web scrape dataset produced by EleutherAI, inspired by WebText \citep{radford2019} and OpenWebTextCorpus \citep{gokaslan2019}.

% \item \textbf{Wikipedia (en)}: The dataset, sourced from the TensorFlow Datasets\footnote{\label{wiki_tf}\url{https://www.tensorflow.org/datasets/catalog/wikipedia\#wikipedia20200301en}}, includes articles from the English Wikipedia as a standard source of high-quality text for language modeling.

% \item \textbf{FreeLaw}: This dataset is derived from the CourtListener platform\footnote{\label{freelaw}\url{https://www.courtlistener.com/}}, part of the Free Law Project, which provides access to legal opinions from federal and state courts in the United States.

% \item \textbf{PubMed Abstracts}: This dataset\footnote{\label{pmc_abst}\url{https://github.com/thoppe/The-Pile-PubMed}} includes abstracts from 30 million publications in PubMed, managed by the National Library of Medicine. It encompasses the significantly limited coverage of full texts in PubMed Central (PMC) and includes MEDLINE abstracts from 1946 to the present day.

% \item \textbf{DeepMind Mathematics}: A collection of mathematical problems from various topics formatted as natural language prompts \citep{saxton2018analysing}. It is included in The Pile to enhance the mathematical ability of the language models \citep{brown2020language}.

% \item \textbf{Project Gutenberg (PG-19)}: This dataset consists of classic Western literature from Project Gutenberg, specifically books published before 1919 \citep{Rae2020Compressive}. It represents distinct styles compared to the more modern Books3 and BookCorpus datasets and is already used for long-distance context modeling.

% \item \textbf{BookCorpus2}: An expanded version of the original BookCorpus \citep{zhu2015}, comprising books by unpublished authors, minimizing overlap with Project Gutenberg and Books3, which include published books. It is commonly used for language model training \citep{radford2018improving}.


% \begin{table}[tbh]
% \centering
% \begin{tabular}{llr}
% \toprule
% \bf Language & \bf Dataset & \bf Tokens (Billions)\\
% \midrule
% English & Pile-CC~\citep{pile} & 25.1\\
% English & Books3~\citep{presser2020} & 25.1\\
% English & ArXiv\textsuperscript{\ref{archive}} & 25.1\\
% English & PubMed Central\textsuperscript{\ref{pmc}} & 25.1\\
% English & OpenWebText2~\citep{radford2019} & 12.5\\
% English & Wikipedia\textsuperscript{\ref{wiki_tf}} & 25.1\\
% English & FreeLaw\textsuperscript{\ref{freelaw}} & 10.4\\
% English & PubMed Abstracts\textsuperscript{\ref{pmc_abst}} & 10.4\\
% English & DM Mathematics~\citep{saxton2018analysing} & 16.7\\
% English & Gutenberg (PG-19)~\citep{Rae2020Compressive} & 18.8\\
% English & BookCorpus2~\citep{zhu2015} & 18.8\\
% English & EuroParl~\citep{koehn2005europarl} & 4.2\\
% English & PhilPapers\textsuperscript{\ref{philp}} & 4.2\\
% English & YoutubeSubtitles\textsuperscript{\ref{yts}} & 3.3\\
% English & NIH ExPorter\textsuperscript{\ref{nihg}} & 3.3\\
% English & Enron Emails~\citep{klimt2004enron} & 3.8\\
% \midrule
% \bf English Total & & \bf 232\\
% \midrule
% Other & GitHub\textsuperscript{\ref{gith}} & 46\\
% \midrule
% \bf Total & & \bf 278\\
% \bottomrule
% \end{tabular}
% \caption{Composition and breakdown of our English and programming code datasets.}
% \label{tab:english:data}
% \end{table}



% \item \textbf{EuroParl} is a multilingual parallel corpus initially introduced for machine translation \citep{koehn2005europarl}, but has also been utilized in several other fields of NLP \citep{groves2006hybridity, vanhalteren2008source, ciobanu2017towards}. The version used in this work consists of the proceedings of the European Parliament in 21 European languages from 1996 until 2012.

% \item \textbf{PhilPapers}: A collection of open-access philosophy publications from the Center for Digital Philosophy, University of Western Ontario.\footnote{\label{philp}\url{https://philpapers.org/}}

% \item \textbf{YouTube Subtitles}: This dataset consists of text from human-generated closed captions on YouTube\footnote{\label{yts}\url{https://github.com/sdtblck/youtube_subtitle_dataset}}. It provides not only multilingual data, but also a variety of content including educational material, popular culture, and natural dialogue.

% \item \textbf{NIH Grant Abstracts}: This dataset includes abstracts of awarded applications from the EXPORTER service, covering fiscal years 1985-present. It was included because it features high-quality scientific writing.\footnote{\label{nihg}\url{https://exporter.nih.gov/}}

% \item \textbf{Enron Emails}: This dataset \citep{klimt2004enron} is widely used for analyzing email usage patterns. It was included to aid in understanding the modality of email communications, which is typically not found in other datasets.

% \item \textbf{GitHub}: This dataset\footnote{\label{gith}\url{https://github.com/EleutherAI/github-downloader}} consists of a large collection of open-source code repositories \citep{brown2020language}. It was included to improve the model's downstream performance on code-related tasks, given GPT-3's ability to generate plausible code completions without any explicitly gathered code datasets.
% \end{itemize}


% Table~\ref{tab:domain:data} summarizes the composition of our dataset: a total of 395B tokens, including Arabic, English, and programming code.


% \begin{table}[htb]
% \centering
% \begin{tabular}{lrrrr}
% \toprule
% \bf Domain & \bf Original & \bf + Translation & \bf + Upsampling & \bf Percentage \\
% \midrule
% Arabic & 55B & 72B & 116B & 29\% \\
% English & 232B & 232B & 232B & 59\% \\
% Programming code & 46B & 46B & 46B & 12\% \\
% \midrule
% \bf Total & & & \bf 395B & \bf 100\%\\
% \bottomrule
% \end{tabular}
% \caption{Distribution of the three primary domains in our mixed pre-training dataset: we first augment the Arabic data by adding 18B translated tokens, and then upsample the resulting Arabic dataset 1.6 times. (\emph{The numbers 72B and 395B are correct, and the summation discrepancies are due to rounding.})}
% \label{tab:domain:data}
% \end{table}

==> commented_text_3.tex <==
% We pretrain the LLM on hundreds of billions of words of diverse text from a variety of sources in order to develop a strong foundation in the target language(s) while at the same time establishing a broad factual knowledge base in the model. In settings such as clinical domains, research has shown that larger-scale LLMs exhibit improved emergent capabilities \citep{singhal2022large}. Note that LLMs such as LLaMA \citep{touvron2023llama} and Falcon \citep{falcon40b} are predominantly trained on a single language: English. While these models exhibit impressive linguistic and reasoning capabilities, their abilities do not extend so well to other languages such as Arabic, as we will demonstrate experimentally below. 

% \begin{table}[tbh]
% \centering
% \begin{tabular}{llr}
% \toprule
% \bf Language & \bf Dataset & \bf Token count \\
% \midrule
% Arabic & Abu El-Khair~\citep{abu2016} & 260,407,899\\
% Arabic & Aranews~\citep{goldhahn2012building} & 203,982,492\\
% Arabic & C4~\citep{raffel2020exploring} & 25,010,967,834\\
% Arabic & ArabicNews 2020 & 1,870,309,674\\
% Arabic & Maktabah\textsuperscript{\ref{Maktabah}} & 1,785,221,183\\
% Arabic & UN~\citep{ziemski-etal-2016-united} & 492,787,444\\
% Arabic & Arabic Wikipedia\textsuperscript{\ref{ArabicWikipedia}
% } & 173,873,517\\
% Arabic & En2Ar Wikipedia & 3,036,944,104 \\
% Arabic & Baai1 (ArabicWeb22-A)\textsuperscript{\ref{ArabicText2022}} & 8,242,639,393\\
% Arabic & Baai2 (ArabicWeb16)~\citep{reem2016} & 5,920,544,065\\
% Arabic & Baai3 (OSCAR)\textsuperscript{\ref{OSCAR}} & 3,331,705,832\\
% Arabic & Baai4 (ArabicWeb22-B)\textsuperscript{\ref{ArabicText2022}} & 2,426,671,361\\
% Arabic & Baai5 (CC100)~\citep{conneau2020} & 2,180,480,535\\
% Arabic & Baai7 (Arabic Tweets)\textsuperscript{\ref{ArabicText2022}} & 210,506,141\\
% Arabic & Misc\textsuperscript{\ref{Misc}} & 31,757,468\\
% \midrule
% \bf Total & & \bf 55,178,798,942\\
% \bottomrule
% \end{tabular}
% \caption{Composition and breakdown of our Arabic pretraining dataset (without translation).}
% \label{tab:arabic:data}
% \end{table}


% Moreover, the extent of knowledge of Arabic world embedded in these models is limited, as they only include relatively small amounts of native Arabic text. To tackle this challenge, we pretrain our model with the largest Arabic dataset in the world, while further extending it with English data and some programming code, to improve the logical reasoning abilities of the model. 

% Our pretraining data mix is 1:2:0.4 for Arabic:English:code. We arrived at this ratio through extensive experiments on smaller models, which we describe in Section~\ref{sec:model}. We base this mix on all of the available Arabic data, as this is the smallest of the three data sources.

% We collect our Arabic training data from multiple sources including web pages, Wikipedia articles, news articles, Arabic books, and social network content. To augment the dataset, we also translate English content to Arabic using an in-house machine translation system.\footnote{Our in-house translation system is a standard transformer sequence-to-sequence model implemented in the FairSeq library~\citep{ott-etal-2019-fairseq} and trained on public datasets available in OPUS~\citep{tiedemann-2012-parallel}. The English to Arabic translation performance is 31 and 40 BLEU points \citep{papineni-etal-2002-bleu} on Flores-101 and a held-out test dataset, respectively.} We restrict this to high-quality English resources such as the English Wikipedia and English books. We apply checks to avoid translating English sources with embedded code, or text that is not well structured.


% A breakdown of the Arabic dataset (except the translated content) is detailed in Table \ref{tab:arabic:data}. Specifically, we use text from the following sources:
% \begin{itemize}
% \item \textbf{Abu El-Khair}: a collection of more than five million news articles, collected from ten major news sources of Arabic countries over a period of fourteen years \citep{abu2016}.

% \item \textbf{Aranews}: Arabic news corpus from multiple sources ranging from year 2005-2022 \citep{goldhahn2012building}

% \item \textbf{ArabicText 2022}: an open-source Arabic collection\footnote{\label{ArabicText2022}\url{https://data.baai.ac.cn/details/ArabicText-2022}} prepared by the Beijing Academy of Artificial Intelligence (BAAI), that includes Arabic text corpora such as ArabicWeb22-A, ArabicWeb16 \citep{reem2016}, OSCAR\footnote{\label{OSCAR}\url{https://oscar-project.org/}}, ArabicWeb22-B, CC100-AR \citep{conneau2020}, and Arabic Tweets. 

% \item \textbf{Arabic subset of C4}: a cleaned version of the Common Crawl using the cleaning and the filtering described in \citep{raffel2020exploring}. We use the Arabic subset of this corpus.

% \item \textbf{Arabic Wikipedia}: Wikipedia written in Arabic\footnote{\label{ArabicWikipedia}\url{https://dumps.wikimedia.org/}}

%  \item \textbf{ArabicNews 2020}: an in-house news crawl at Inception of various Arabic news channels.

%  \item \textbf{Maktabah}: a corpus of approximately 6,500 Arabic books.\footnote{\label{Maktabah}\url{https://www.kaggle.com/datasets/mahmoudqaddoumi/arabic-library}}
%  \item \textbf{UN Meeting transcripts}: the United Nations Parallel Corpus,\footnote{\url{https://conferences.unite.un.org/uncorpus}} v1.0 \citep{ziemski-etal-2016-united} which is available in the six official languages of the United Nations, of which we use the Arabic documents. 

% \item \textbf{Other Sources}: a combined dataset of multiple smaller corpora including poetry, news, entertainment, sports, and management documents.\footnote{\label{Misc}\url{https://master.dl.sourceforge.net}, \url{https://github.com/ceefour/hadith-islamware}, \url{https://alt.qcri.org/resources1/qedcorpus/QEDCorpusv1.4_MT.tgz}}
% \end{itemize}  


% We further augment the Arabic data by translating  3B tokens from English Wikipedia and 15B tokens from the Books3 corpus. As a result, we increase the Arabic data from 55B to 72B tokens. Subsequently, we upsample this Arabic data 1.6 times, obtaining 116B Arabic tokens.

% For English, we use The Pile \citep{pile}, a collection of 22 high-quality datasets, from which we randomly sample 232B English tokens and 46B tokens from its GitHub subset. Table~\ref{tab:english:data} shows details about the English data we use. Specifically, we use text from the following sources, part of The Pile:


% \begin{itemize}

% \item \textbf{Pile-CC}: A subset of The Pile dataset, derived from the Common Crawl, a collection of website crawls from 2008 onwards. The dataset includes raw web pages, metadata, and text extractions from diverse domains. Due to the varying quality of the data in Common Crawl, Pile-CC is created using jusText \citep{endredy2013more} on Web Archive files for extraction, yielding higher quality output than directly using the WET files \citep{pile}.

% \item \textbf{Books3}: Derived from the contents of the Bibliotik private tracker made available by Shawn Presser \citep{presser2020}. It is a mix of fiction and non-fiction books, significantly larger than the next largest dataset, BookCorpus2, and was included for its value in long-range context modeling and coherent storytelling.

% \item \textbf{ArXiv}: A subset of the ArXiv preprint repository for research papers, which has been in operation since 1991.\footnote{\label{archive}\url{https://arxiv.org/}}

% \item \textbf{PubMed Central}: A subset of the PubMed online repository for biomedical articles, managed by the United States' National Center for Biotechnology Information (NCBI).\footnote{\label{pmc}\url{https://www.ncbi.nlm.nih.gov/pmc}}

% \item \textbf{OpenWebText2}: A web scrape dataset produced by EleutherAI, inspired by WebText \citep{radford2019} and OpenWebTextCorpus \citep{gokaslan2019}.

% \item \textbf{Wikipedia (en)}: The dataset, sourced from the TensorFlow Datasets\footnote{\label{wiki_tf}\url{https://www.tensorflow.org/datasets/catalog/wikipedia\#wikipedia20200301en}}, includes articles from the English Wikipedia as a standard source of high-quality text for language modeling.

% \item \textbf{FreeLaw}: This dataset is derived from the CourtListener platform\footnote{\label{freelaw}\url{https://www.courtlistener.com/}}, part of the Free Law Project, which provides access to legal opinions from federal and state courts in the United States.

% \item \textbf{PubMed Abstracts}: This dataset\footnote{\label{pmc_abst}\url{https://github.com/thoppe/The-Pile-PubMed}} includes abstracts from 30 million publications in PubMed, managed by the National Library of Medicine. It encompasses the significantly limited coverage of full texts in PubMed Central (PMC) and includes MEDLINE abstracts from 1946 to the present day.

% \item \textbf{DeepMind Mathematics}: A collection of mathematical problems from various topics formatted as natural language prompts \citep{saxton2018analysing}. It is included in The Pile to enhance the mathematical ability of the language models \citep{brown2020language}.

% \item \textbf{Project Gutenberg (PG-19)}: This dataset consists of classic Western literature from Project Gutenberg, specifically books published before 1919 \citep{Rae2020Compressive}. It represents distinct styles compared to the more modern Books3 and BookCorpus datasets and is already used for long-distance context modeling.

% \item \textbf{BookCorpus2}: An expanded version of the original BookCorpus \citep{zhu2015}, comprising books by unpublished authors, minimizing overlap with Project Gutenberg and Books3, which include published books. It is commonly used for language model training \citep{radford2018improving}.


% \begin{table}[tbh]
% \centering
% \begin{tabular}{llr}
% \toprule
% \bf Language & \bf Dataset & \bf Tokens (Billions)\\
% \midrule
% English & Pile-CC~\citep{pile} & 25.1\\
% English & Books3~\citep{presser2020} & 25.1\\
% English & ArXiv\textsuperscript{\ref{archive}} & 25.1\\
% English & PubMed Central\textsuperscript{\ref{pmc}} & 25.1\\
% English & OpenWebText2~\citep{radford2019} & 12.5\\
% English & Wikipedia\textsuperscript{\ref{wiki_tf}} & 25.1\\
% English & FreeLaw\textsuperscript{\ref{freelaw}} & 10.4\\
% English & PubMed Abstracts\textsuperscript{\ref{pmc_abst}} & 10.4\\
% English & DM Mathematics~\citep{saxton2018analysing} & 16.7\\
% English & Gutenberg (PG-19)~\citep{Rae2020Compressive} & 18.8\\
% English & BookCorpus2~\citep{zhu2015} & 18.8\\
% English & EuroParl~\citep{koehn2005europarl} & 4.2\\
% English & PhilPapers\textsuperscript{\ref{philp}} & 4.2\\
% English & YoutubeSubtitles\textsuperscript{\ref{yts}} & 3.3\\
% English & NIH ExPorter\textsuperscript{\ref{nihg}} & 3.3\\
% English & Enron Emails~\citep{klimt2004enron} & 3.8\\
% \midrule
% \bf English Total & & \bf 232\\
% \midrule
% Other & GitHub\textsuperscript{\ref{gith}} & 46\\
% \midrule
% \bf Total & & \bf 278\\
% \bottomrule
% \end{tabular}
% \caption{Composition and breakdown of our English and programming code datasets.}
% \label{tab:english:data}
% \end{table}



% \item \textbf{EuroParl} is a multilingual parallel corpus initially introduced for machine translation \citep{koehn2005europarl}, but has also been utilized in several other fields of NLP \citep{groves2006hybridity, vanhalteren2008source, ciobanu2017towards}. The version used in this work consists of the proceedings of the European Parliament in 21 European languages from 1996 until 2012.

% \item \textbf{PhilPapers}: A collection of open-access philosophy publications from the Center for Digital Philosophy, University of Western Ontario.\footnote{\label{philp}\url{https://philpapers.org/}}

% \item \textbf{YouTube Subtitles}: This dataset consists of text from human-generated closed captions on YouTube\footnote{\label{yts}\url{https://github.com/sdtblck/youtube_subtitle_dataset}}. It provides not only multilingual data, but also a variety of content including educational material, popular culture, and natural dialogue.

% \item \textbf{NIH Grant Abstracts}: This dataset includes abstracts of awarded applications from the EXPORTER service, covering fiscal years 1985-present. It was included because it features high-quality scientific writing.\footnote{\label{nihg}\url{https://exporter.nih.gov/}}

% \item \textbf{Enron Emails}: This dataset \citep{klimt2004enron} is widely used for analyzing email usage patterns. It was included to aid in understanding the modality of email communications, which is typically not found in other datasets.

% \item \textbf{GitHub}: This dataset\footnote{\label{gith}\url{https://github.com/EleutherAI/github-downloader}} consists of a large collection of open-source code repositories \citep{brown2020language}. It was included to improve the model's downstream performance on code-related tasks, given GPT-3's ability to generate plausible code completions without any explicitly gathered code datasets.
% \end{itemize}


% Table~\ref{tab:domain:data} summarizes the composition of our dataset: a total of 395B tokens, including Arabic, English, and programming code.


% \begin{table}[htb]
% \centering
% \begin{tabular}{lrrrr}
% \toprule
% \bf Domain & \bf Original & \bf + Translation & \bf + Upsampling & \bf Percentage \\
% \midrule
% Arabic & 55B & 72B & 116B & 29\% \\
% English & 232B & 232B & 232B & 59\% \\
% Programming code & 46B & 46B & 46B & 12\% \\
% \midrule
% \bf Total & & & \bf 395B & \bf 100\%\\
% \bottomrule
% \end{tabular}
% \caption{Distribution of the three primary domains in our mixed pre-training dataset: we first augment the Arabic data by adding 18B translated tokens, and then upsample the resulting Arabic dataset 1.6 times. (\emph{The numbers 72B and 395B are correct, and the summation discrepancies are due to rounding.})}
% \label{tab:domain:data}
% \end{table}

==> commented_text_4.tex <==
% Large language models (LLMs) have revolutionized the field of natural language processing (NLP), demonstrating remarkable capabilities in generating high-quality texts and resulting in widespread adoption across a diverse array of practical NLP applications and domains.
% Yet, the main focus of research and development efforts so far has been on English. While recent LLMs such as Falcon \citep{falcon40b}, PALM \citep{chowdhery2022palm} and LLaMA \citep{touvron2023llama,touvron2023llama2}, among others, are able to process data in multiple languages, they were nevertheless primarily trained and instruction-tuned for English. As a result, they are not able to extend their understanding and generation capabilities to languages other than English. In this work, we aim to bridge this gap. We focus on Arabic, one of the world's most spoken languages with over 400M speakers, which has been noticeably underrepresented in the LLM  space so far. In particular, we develop \modelname{}, a powerful Arabic-centric decoder-only LLM with 13B parameters, based on the GPT-3 generative pretraining architecture~\citep{brown2020language}. 

% The primary challenge in developing an Arabic LLM is the limited availability of high-quality Arabic data. As compared to English, where corpora of size up to two trillion tokens are readily available \citep{touvron2023llama2}, Arabic corpora are significantly smaller in size. As part of this work, we have collected the largest Arabic corpora to date, consisting of 72 billion tokens. However, this dataset is still not sufficiently large for the purposes of training an Arabic LLM capable of demonstrating emergent capabilities \citep{openai2023gpt4}. 

% To address this, we train bilingual models, by augmenting the limited Arabic pretraining data with abundant English pretraining data. We pretrain \modelname{} on 395 billion tokens, including 72 billion Arabic tokens (which we repeat 1.6 times, to obtain an effective total of 116 billion Arabic tokens), 232 billion English tokens, and the remainder being code in various programming languages. As part of our effort, we have designed and developed a specialized Arabic text processing pipeline that includes thorough data filtering and cleaning to produce high-quality Arabic data.

% Unlike previous massively multilingual LLMs such as BLOOM~\citep{Scao2022BLOOMA1} or mT0 \citep{muennighoff2022crosslingual}, which contain more than 50 languages, we do not include languages aside from Arabic and English in any significant percentage. Neither do we relegate Arabic to a minority in the pretraining dataset. Instead, Arabic data constitutes 33\% of our pretraining. Our choice of mixing two languages attains the best of both worlds; the LLM is highly fluent in Arabic, with linguistic capability as well as cultural awareness and sensitivity. At the same time, it is on par with recent English LLMs in terms of reasoning capacity and world knowledge, capabilities we observe to have transferred from English to Arabic and vice-versa.

% Building upon the standard transformer architecture \citep{vasava-etal-2022-transformer} in the form of its GPT-3 variant, we adopt a number of improvements from the literature including (\emph{i})~ALiBi \citep{alibi} positional encodings, which enable the model to extrapolate to longer contexts at inference, (\emph{ii})~SwiGLU activation function \citep{shazeer2020gluvariants} to improve the performance, (\emph{iii})~maximal update parametrization to perform hyperparameter optimization based on experiments with smaller models \citep{yang2022mup}, and (\emph{iv})~a custom-built tokenizer that weighs both languages equally.

% We further develop an instruction-tuned version of our model, \modelnametuned{}, which uses over 3.6 million Arabic and 6 million English instruction-response pairs. Considering the inherent safety concerns of LLMs, we further fine-tune it with safety-oriented instructions. In our deployed system which provides an interactive interface to the instruction-tuned model \footnote{\url{https://arabic-gpt.ai}}, we add extra guardrails in the form of safety prompts, keyword-based filtering, and external classifiers. An example conversation with \modelnametuned{} on this interface is shown in Figure~\ref{fig:dialog:example}.


% We evaluate \modelname{} and \modelnametuned{} across a wide array of Arabic and English NLP benchmarks, addressing reasoning, knowledge, misinformation, and bias. The results show that \modelname{} is superior in Arabic compared to other models of similar size, while also being competitive in English, despite being trained on significantly less English data.

% We are releasing the following models:

% \begin{itemize}
%     \item \modelname{}\footnote{\url{https://huggingface.co/inception-mbzuai/jais-13b}}: base pretrained 13B foundation model;
%     \item \modelnametuned{}\footnote{\url{https://huggingface.co/inception-mbzuai/jais-13b-chat}}: instruction-tuned 13B version of \modelname{}, optimized for dialog interaction.
% \end{itemize}

% By making our models publicly available, we hope to enable further research and development in this area, stimulating innovation and practical applications that can better serve the Arabic and the global communities. Despite our significant efforts to ensure safety, we recognize that the models are not foolproof and may not cover all cases. Therefore, we strongly urge all adopters to exercise caution and to conduct additional safety testing before deploying our models. For this purpose, we outline responsible release notes in Section \ref{sec:release}.


% \begin{figure}[t!]
%     \centering
%     \includegraphics[width=\columnwidth]{figures/rent_big_b}
%     \caption{English--Arabic multiturn dialogue using \modelnametuned{}.}
%     \label{fig:dialog:example}
% \end{figure}

==> commented_text_5.tex <==

\section{Related Work [MBZUAI] <Amr>}
\label{sec:related}

\paragraph{Large Language Models.} Large Language Models (LLMs) have demonstrated strong performance across tasks and languages (CITATION). Multilingual models have enabled cross-lingual transfer over the different languages, with early text-to-text systems—such as \textit{mT5}—having shown that scaling multilingual pretraining improves zero-shot generalization across scripts \citep{xue2020mt5}. More recent work (e.g., \textit{Llama 3}) has combined large, curated, and de-duplicated multilingual corpora with refined tokenization and broad multilingual evaluation \citep{grattafiori2024llama3herdmodels}. Despite these advances, generic tokenizers and data mixtures have often underrepresented low-resource languages---notably Arabic, with its rich morphology and substantial dialectal variation---thereby motivating targeted bilingual and Arabic-centric modeling approaches.

\paragraph{Arabic Language Models.} In response to these gaps, a wave of Arabic-centric and bilingual LLMs has emerged. \textit{Jais} introduced a bilingual Arabic--English pretraining recipe with carefully curated Arabic corpora and Arabic-oriented instruction tuning, reporting strong results on Arabic understanding and generation benchmarks; this effort was later extended by \textit{Jais-adapted}, which applied continual pretraining and post-training on a strong English backbone to enhance Arabic fluency and robustness to dialectal variation while preserving English performance \citep{sengupta2023jaisjaischatarabiccentricfoundation,gosal2024bilingual}. Open releases further expanded the ecosystem: \textit{AceGPT} provided instruction-tuned Arabic models with cultural alignment, \textit{ALLaM} introduced bilingual Arabic–English models emphasizing cross-lingual knowledge transfer and alignment for improved Arabic and English performance, and \textit{Fanar} developed LLM variants optimized for Arabic instruction following, trained on a mixed corpus of Arabic, English, and code data \citep{huang-etal-2024-acegpt,bariallam,fanarllm2025}. Collectively, these efforts underscore the value of Arabic-aware tokenization, balanced bilingual data mixtures, and culturally grounded instruction tuning; yet comprehensive coverage across dialects, morphology, and orthographic variation remains open, motivating continued progress on next-generation Arabic and bilingual LLMs. Parallel lines of work have also explored dialect-specialized modeling—e.g., \textit{Nile-Chat} for Egyptian Arabic and \textit{Atlas-Chat} for Moroccan Darija—which train and evaluate directly on dialectal corpora (often across Arabic and Latin/Arabizi scripts). While these works advance dialectal competence, they largely develop dialect models in isolation from MSA and seldom provide unified MSA–dialect instruction-tuning resources spanning both scripts, leaving joint coverage and cross-varietal transfer underexplored \citep{shang2025nilechategyptianlanguagemodels,shang2024atlaschatadaptinglargelanguage}.

\paragraph{Instruction Fine-Tuning.} Instruction fine-tuning (IFT) adapts next-token–trained LLMs to follow natural-language instructions by supervising on prompt–response pairs and, in some cases, optimizing with human preference signals. Early work (often termed SFT+RLHF) established the paradigm of supervised instruction data followed by preference-based alignment \citep{ouyang2022training}. Subsequent efforts showed that high-quality supervised instruction corpora alone can yield strong instruction following \citep{wei2021finetuned,wang2023self,alpaca}. Preference-optimization approaches such as Direct Preference Optimization (DPO) later simplified alignment by replacing online RL with a purely supervised objective on ranked pairs \citep{rafailov2023dpo}.

General-purpose instruction datasets span task- and domain-diverse mixtures (classification, reasoning, math, code, dialogue) and increasingly emphasize multi-turn structure, safety, and evaluation-ready formatting. Examples include Super-NaturalInstructions and prompted mixtures like P3/xP3 for cross-lingual coverage \citep{wang2022super,muennighoff2022crosslingual}, as well as synthetic instruction sets designed to stress-test generalization (e.g., Unnatural Instructions) \citep{honovich2023unnatural}. Recent open instruction pipelines further highlight the importance of careful deduplication, contamination control, and response-quality filtering for robust IFT \citep{lambert2025tulu3pushingfrontiers}.

Multilingual IFT has advanced along two complementary tracks: (i) native, human-authored supervision in many languages, and (ii) translation-augmented instruction sets to reach low-resource settings. Collections such as xP3 and Aya broaden instruction coverage across dozens to 100+ languages and scripts, enabling zero-/few-shot transfer and cross-lingual consistency \citep{muennighoff-etal-2023-crosslingual,singh2024ayadatasetopenaccesscollection}. Nevertheless, many multilingual mixtures still lean heavily on translated English sources, which can propagate cultural and stylistic biases and under-represent dialectal phenomena.

Arabic-centric IFT has emerged to address these gaps. Recent releases—e.g., \textit{Jais} and \textit{Jais-adapted}, \textit{Allam}, \textit{AceGPT}, and \textit{Fanar}—adopt bilingual or Arabic-first curation strategies, mix native Arabic with translated instruction data, and explore evaluation tailored to Arabic tasks \citep{sengupta2023jaisjaischatarabiccentricfoundation,gosal2024bilingual,bariallam,huang-etal-2024-acegpt,fanarllm2025}. However, most prior Arabic IFT pipelines emphasize MSA and broad utility tasks, with comparatively limited emphasis on dialectal coverage across scripts, culturally grounded domains, and domain-specific reasoning datasets in Arabic (e.g., finance). In parallel, dialect-focused efforts have begun releasing public IFT corpora for Egyptian Arabic and Moroccan Darija—often in both Arabic and Latin (Arabizi) scripts—such as \textit{Nile-Chat} and \textit{Atlas-Chat}.

Building on this line of work, we pursue a bilingual (Arabic–English) IFT strategy that (a) couples high-quality open IFT corpora with carefully translated augmentation where native Arabic is scarce, (b) explicitly targets dialectal diversity (e.g., Egyptian and Moroccan Darija in Arabic and Latin scripts), and (c) adds culturally grounded and domain-focused Arabic instruction sets (poetry, dream interpretation, cuisine, finance QA and summarization, dialect identification).

\paragraph{Evaluating Large Language Models.}
Recent efforts evaluate LLMs along three axes: (i) downstream knowledge and reasoning using suites like \textit{MMLU}, \textit{HellaSwag}, and \textit{ARC} \citep{hendrycks2020measuring,zellers-etal-2019-hellaswag,clark2018think}; (ii) instruction following and open-ended generation via LLM-as-a-judge protocols (Vicuna-style) and Arabic-focused \textit{AraGen} with its 3C3H rubric, plus \textit{Arabic IFEval} for strict instruction compliance \citep{vicuna,aragen,ifeval}; and (iii) safety and bias with culturally aware audits such as the \textit{Arabic LLM Safeguard Evaluation} \citep{ashraf-etal-2025-arabic}. Most Arabic evaluations still rely on translated English sets, with limited dialect coverage and domain breadth. In this work, we complement standard suites with standard suites with \textit{Arabic-native}, dialect- and script-aware evaluations—spanning poetry, cuisine (ACB), Islamic QA, and finance. We contribute new MCQ and generative test sets, and instruction-compliance reporting with targeted human verification and region-aware safety auditing, improving cultural fidelity and reproducibility.

% \subsection{Recent Work on Data Mixing}
% \label{sec:realted_mixing}
% \todo{[Preslav] This appears to be just copied from another paper. Check!}

% Contemporary foundation models have validated this approach. OLMo 2 \citep{olmo20252olmo2furious} introduces a systematic methodology for developing data mixes through iterative ablation, employing a ``microannealing'' procedure that rapidly evaluates candidate data sources by training on 100\% of their content to assess performance impact. Llama 3 \citep{grattafiori2024llama3herdmodels} employs a related but distinct strategy, incorporating data annealing where harder, higher-quality data (particularly mathematical reasoning and multilingual content) is preferentially sampled later in pretraining with reduced learning rates. This timing-based approach demonstrates that the order of data presentation interacts non-trivially with the learning rate schedule, with implications for both final performance and training dynamics.




%\end{itemize}
% Below, we discuss previous work on the following relevant topics: Arabic language models, LLMs in general, instruction-tuning, and evaluation of LLMs.

% \paragraph{Arabic Language Models}

% Arabic language models have been developed across various architectures and learning objectives. Examples of encoder-only models include AraBERT \cite{antoun2020arabert}, QARiB \cite{abdelali2021pre}, JABER and SABER\cite{ghaddar2022jaber}, CAMeLBERT \cite{inoue2021interplay}, AraELECTRA 
% \cite{antoun2020araelectra}, GigaBERT \cite{lan2020gigabert}, and ARBERT \& MARBERT \cite{abdul2020arbert}.
% There have been also decoder-only models such as ARAGPT2 \cite{antoun2020aragpt2}. In the encoder--decoder category, prominent models include AraT5 \cite{nagoudi-etal-2022-arat5} and AraBART \cite{eddine2022arabart}. These models, when fine-tuned, have demonstrated competitiveness in both natural language understanding and natural language generation tasks. 

% However, to the best of our knowledge, no public Arabic language model has been trained with over a billion parameters, capable of showcasing generalization and robust zero-shot capabilities across various tasks.\footnote{JASMINE \cite{nagoudi2022jasmine} are Arabic GPT models ranging in sizes from 350M to 13B parameters, but these models have not been released to the public, and the arXiv paper describing them says the 6.7B and 13B models are still training.}
% In addition to monolingual models, Arabic has also been integrated into multilingual models, including earlier models such as mBERT~\cite{devlin2018bert} and XLM-RoBERTa~\cite{conneau2020}, as well as more recent large language models such as BLOOM~\cite{Scao2022BLOOMA1}. However, due to the Arabic content being dwarfed by other languages, these models tend to perform substantially worse than dedicated monolingual models and often exhibit limited generalization abilities in zero-shot settings~\cite{li2023bactrianx}.

% \paragraph{Large Language Models}

% Language models with ever larger numbers of parameters have consistently improved over smaller models such as BERT \cite{devlin2018bert}, BART \cite{lewis2019bart}, and T5 \cite{raffel2020exploring}. Despite their extensive training on multilingual text data, recent large language models have an English-centric bias and are less effective for languages beyond English~\cite{li2023bactrianx}. 
% An exception to this trend is GLM~\cite{zeng2022glm}, which is the sole large language model specifically designed to excel in both Chinese and English. 

% Existing pretraining frameworks for language models fall into three categories: autoregressive, autoencoding, and encoder--decoder models. Most recent large language models, such as the GPT series~\cite{radford2019,brown2020language,openai2023gpt4}, LLaMA \cite{touvron2023llama,touvron2023llama2}, BLOOM~\cite{Scao2022BLOOMA1}, and Falcon \cite{falcon40b}, are autoregressive, using a left-to-right language model objective. Earlier models such as BERT \cite{devlin2018bert}, ELECTRA \cite{clark2019electra}, and RoBERTa~\cite{liu2019roberta} are encoder-only, while BART~\cite{lewis2019bart} and T5~\cite{raffel2020exploring} are encoder--decoder models. As elaborated in Section~\ref{sec:model_arc}, \modelname{} and \modelnametuned{} follow the autoregressive model paradigm, building upon the successes of LLaMA2 and GPT-4. 

% Progress in large language models can also be categorized into two streams: closed-source and open-source models. Closed-source models such as Bard,\footnote{\url{https://ai.google/static/documents/google-about-bard.pdf}} Claude,\footnote{\url{https://www.anthropic.com/index/introducing-claude}} Gopher~\cite{rae2022scaling}, and GPT-4~\cite{openai2023gpt4} offer fewer advantages to the research community compared to open-source models \cite{touvron2023llama2,Scao2022BLOOMA1}. The lack of model transparency exposes leads to various risks for closed-source models, including privacy concerns \cite{mireshghallah-etal-2022-quantifying,yermilov-etal-2023-privacy} and safety issues \cite{sun-etal-2022-safety}. In contrast, \modelname{} and \modelnametuned{} are open-source models, as elaborated in Section~\ref{sec:model}.


% \paragraph{Instruction-Tuning}

% Fine-tuning language models using instruction--response pairs has enhanced the generalization capabilities of language models across various tasks \cite{ouyang2022training}. In terms of open-source models, BLOOMz \cite{muennighoff2022crosslingual} is a fine-tuned version of the foundation model BLOOM \cite{Scao2022BLOOMA1} based on large-scale instruction-tuning over a dataset created via templates, while LLaMA2~\cite{touvron2023llama2} uses a publicly available instruction--response pair dataset \cite{chung2022scaling}. Moreover, instruction-tuning has been coupled with reinforcement learning with human feedback (RLHF). This combination aligns the generated responses to reward functions, optimizing the model's factuality, and reducing its toxicity \cite{ouyang2022training}.


% The prompts used for instruction-tuning can have diverse origins. Some, as observed by \cite{zhou2023large}, are human-designed, while others can be autonomously generated. These prompts can be refined with follow-up instructions for more relevant or specific outputs, as studied by \cite{ganguli2023capacity} and \cite{madaan2023selfrefine}. Recently, \cite{wei2023chainofthought} introduced \emph{chain-of-thought prompting}, directing models to clarify their reasoning over complex tasks, which was shown to enhance their accuracy.



% \paragraph{Evaluating Large Language Models}

% Large language models are proficient at generating coherent and fluent text, but have shortcomings in terms of factuality and reasoning skills. As a proxy to evaluate factuality, existing English large language models such as GPT-4~\cite{openai2023gpt4} and LLaMA~\cite{touvron2023llama} use school exam questions~\cite{hendrycksmeasuring} to understand how faithful the models are at providing knowledge. Evaluating commonsense reasoning abilities is also important, and is the target of datasets such as \emph{HellaSwag}~\cite{zellers-etal-2019-HellaSwag}, \emph{WinoGrande}~\cite{sakaguchi2021winogrande}, \emph{ARC} easy and challenge~\cite{clark2018think}, and \emph{OpenBookQA}~\cite{mihaylov-etal-2018-suit}. Moreover, reasoning via programming is evaluated using HumanEval~\cite{chen2021evaluating} and
% MBPP~\cite{austin2021program}. 

% In Arabic NLP, existing benchmarks primarily focus on evaluating natural language understanding tasks. For instance, the ALUE benchmark~\cite{seelawi-etal-2021-alue} encompasses semantic tasks such as irony detection \cite{ghanem2019idat}, emotion classification \cite{mohammad-etal-2018-semeval}, sentiment classification \cite{mohammad-etal-2018-semeval}, offensive language~\cite{mubarak-etal-2020-overview} and hate speech identification~\cite{mubarak-etal-2020-overview}.
% Existing Arabic benchmarks, however, do not include knowledge and commonsense evaluation, posing a challenge for the assessment of \modelname{}. 

% In contrast, in other languages, researchers have effectively used methods such as machine translation or the construction of datasets in a similar manner to assess the knowledge proficiency and the commonsense understanding of language models \cite{openai2023gpt4,li2023bactrianx}.
% In this context, as detailed in Section~\ref{sec:Evaluation}, we used a combination of techniques, including crafting analogous datasets to those available for English, using human translations and our in-house machine translation system to convert English datasets into Arabic for the purposes of evaluation.

% Evaluating only on knowledge \cite{hendrycksmeasuring,li2023cmmlu} and commonsense reasoning \cite{zellers-etal-2019-HellaSwag,sakaguchi2021winogrande} based on the evaluation settings of prior work \cite{touvron2023llama,muennighoff2022crosslingual} is arguably not a holistic evaluation, as they are multiple-choice questions. To evaluate the generated text as a whole, human evaluation remains crucial. Unfortunately, it is both resource-intensive and sometimes exhibits variable quality, especially when using crowd-sourcing. Recent studies \cite{tornberg2023chatgpt,luo2023chatgpt,gao2023human, wu2023style} have even suggested that ChatGPT annotation surpasses the performance of Amazon crowd-sourced workers, underscoring the importance of expert workers in the evaluation process. Expanding upon these findings, another study~\cite{peng2023instruction,vicuna} used GPT-4 as a substitute for crowd-sourced workers to compare two model outputs. This is achieved by presenting an evaluation prompt and providing both model outputs as a context for the assessment.




==> data_decontamination.tex <==
Data contamination or leakage between training and evaluation datasets can lead to inflated performance metrics, as models may reproduce information they have previously encountered instead of demonstrating genuine generalization. To ensure that our assessments accurately reflect true model capability, we apply data decontamination to both our Instruction-Finetuning (IFT) and benchmark datasets. To achieve this, we developed our own data decontamination pipeline, which systematically identifies and removes overlapping or near-duplicate examples. This approach allows us to maintain the integrity and reliability of our evaluations while ensuring that our benchmarks measure genuine model understanding rather than memorization.

\begin{figure}[H]
    \centering
    \includegraphics[width=1\linewidth]{figures/Data_Decontamination_Pipeline.pdf}
    \caption{Data decontamination pipeline consisting of 3 experts.}
    \label{fig:data_decontamination_pipeline}
\end{figure}

\subsection{Pipeline Overview}
Inspired by prior work \citep{touvron2023llama2openfoundation, yang2023rethinking}, we developed the pipeline illustrated in Figure~\ref{fig:data_decontamination_pipeline} to assess data using both semantic and syntactic similarity measures, which we refer to as the semantic and syntactic judges. Because each judge may produce a substantial number of false positives, we incorporate an additional decontamination stage—LLM-as-a-judge—to validate whether the combined outputs of these judges correspond to true positives.

\subsection{N-Gram Similarity}
% Our approach employs a high-precision, variable-length \textit{n}-gram matching method to detect data contamination between the training set (IFT) and benchmark datasets. Unlike traditional fixed-length \textit{n}-gram analysis, which uses a constant window size (e.g., $N = 13$), our method dynamically adjusts the window length across a range of values to capture both short, specific overlaps and long, verbatim matches. By iteratively generating and comparing \textit{n}-grams for each document over lengths $L = \text{min\_len}, \text{min\_len}+1, \ldots,$ up to the full sequence, the algorithm avoids the blind spots of fixed-window approaches, ensuring that subtle phrase-level similarities and extended copied segments are both detected accurately.

Our approach employs a fixed-length \textit{n}-gram matching method to detect data contamination between the training set (IFT) and benchmark datasets. We use a fixed \textit{n}-gram size (e.g., $n = 4$) and exhaustively compare all contiguous \textit{n}-grams in the IFT documents against those in the benchmark. This design yields a precise detector of phrase-level overlap, while remaining computationally efficient and easy to interpret.


\subsection{Embedding Similarity}
We adopt a straightforward similarity pipeline. We first encode all benchmark and IFT samples into vector representations using the chosen embedding model, and then compute cosine similarity between every IFT embedding and the benchmark embeddings (via a FAISS index). For texts that exceed the model’s maximum input length, we apply a sliding window over the tokenized sequence, embed each window independently, and use the mean of the window embeddings as the representation of the full text. This chunk-and-average strategy allows us to handle long documents while remaining compatible with standard fixed-length embedding models.


\subsection{LLM-as-a-Judge}
Manual inspection revealed that each expert tends to produce a substantial number of false positives, particularly for very long documents or texts written in diverse dialects. To mitigate this issue, we introduce an additional verification stage using an LLM-as-a-judge. All candidate overlaps identified by either expert are passed to this judge model, which determines whether they constitute genuine contamination.

\subsection{Hyperparameters}
To select effective hyperparameters, we first surveyed public leaderboards and identified state-of-the-art models for each component of our pipeline. We then evaluated multiple candidate models and threshold settings on internally labeled datasets to determine an optimal configuration. In this process, we prioritized high recall to ensure a conservative, safety-oriented decontamination procedure. The final setup achieved an average recall exceeding 90\%.

For the embedding-similarity stage, we selected the Arabic embedding model \model{GATE-AraBert-v1}\footnote{\url{https://huggingface.co/Omartificial-Intelligence-Space/GATE-AraBert-v1}}
 with a similarity threshold of 80\%, meaning that any pair with cosine similarity above this threshold is treated as potentially contaminated. For the \textit{n}-gram stage, we chose a conservative 20\% overlap threshold with $n=4$, which corresponds to very low surface-form similarity but aligns with our goal of being maximally cautious. Finally, for the judge layer, we used \model{gemma-3-12b-it}\footnote{\url{https://huggingface.co/google/gemma-3-12b-it}}
 to adjudicate the candidate contamination pairs produced by the previous stages.

